From Sound Workflow Nets to LTLf Declarative Specifications by Casting Three Spells

In process management, effective behavior modeling is essential for understanding execution dynamics and identifying potential issues. Two complementary paradigms have emerged in the pursuit of this objective: the imperative approach, representing all allowed runs of a system in a graph-based model, and the declarative one, specifying the rules that a run must not violate in a constraint-based specification. Extensive studies have been conducted on the synergy and comparisons of the two paradigms. To date, though, whether a declarative specification could be systematically derived from an imperative model such that the original behavior was fully preserved (and if so, how) remained an unanswered question. In this paper, we propose a three-fold contribution. (1) We introduce a systematic approach to synthesize declarative process specifications from safe and sound Workflow nets. (2) We prove behavioral equivalence of the input net with the output specification, alongside related guarantees. (3) We experimentally demonstrate the scalability and compactness of our encoding through tests conducted with synthetic and real-world testbeds.

==> addon/glossary.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CUSTOMISE THIS FILE as you please
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Acronyms / abbreviations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keywords
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Variables
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%


==> addon/macros-DECLARE-drawing.tex <==
% for file in *.tex; do echo ${file%.*} | sed -e 's/^\(.\)/Draw\u\1/' | sed -e 's/\(.*\)/\\NewDocumentCommand{\\1}{ O{\$\\paramx\$} O{\$\\paramy\$} }{%/'; more "$file" | sed -e 's/\$\\paramx\$/#1/' | sed -e 's/\$\\paramy\$/#2/'; echo '%'; echo '}'; echo;  done > ../draw-Declare-macros.tex
\RequirePackage{xparse}

\NewDocumentCommand{\DrawAbsence}{ +O{$\paramx$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center)]\node[DECLARE.task,DECLARE.existcon=$0..m$]{#1};\end{tikzpicture}%
}

\NewDocumentCommand{\DrawAltprec}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.alt.prec] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawAltresp}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.alt.resp] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawAltsucc}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.alt.succ] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawAtmostone}{ O{$\paramx$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center)]\node[DECLARE.task,DECLARE.existcon=$0..1$]{#1};\end{tikzpicture}%
}

\NewDocumentCommand{\DrawChnprec}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.chn.prec] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawChnresp}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.chn.resp] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawChnsucc}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.chn.succ] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawCoex}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.coex] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawEnd}{ O{$\paramx$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center)]\node[DECLARE.task,DECLARE.existcon=End]{#1};\end{tikzpicture}%
}

\NewDocumentCommand{\DrawExistence}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center)]\node[DECLARE.task,DECLARE.existcon=$n..\ast$]{#1};\end{tikzpicture}%
}

\NewDocumentCommand{\DrawInit}{ O{$\paramx$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center)]\node[DECLARE.task,DECLARE.existcon=Init]{#1};\end{tikzpicture}%
}

\NewDocumentCommand{\DrawNotchnsucc}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.chn.succ,DECLARE.neg] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawNotcoex}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.coex,DECLARE.neg] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawNotsucc}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.succ,DECLARE.neg] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawParticipation}{ O{$\paramx$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center)]\node[DECLARE.task,DECLARE.existcon=$1..\ast$]{#1};\end{tikzpicture}%
}

\NewDocumentCommand{\DrawPrec}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.prec] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawResex}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.resex] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawResp}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.resp] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawSucc}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.succ] node {} (2);
\end{tikzpicture}%
}

==> addon/macros-for-requirements-description-list.tex <==
%
% This one allows us to have a custom DESCRIPTION environment, in which numbers are preceded by a one-letter prefix.
% A short description can be added as an additional parameter to the begin-environment command.
% Successive references will have that very one-letter prefix + number with hyper-reference to it.
%
\RequirePackage{enumitem}
%
\def\requiprefix{R}
%
\newcounter{requicount}
\newlist{requidescr}{description}{1}
\setlist[requidescr,1]{%
	before={\setcounter{requicount}{0}%
		\renewcommand*\therequicount{\arabic{requicount}}},
	,font=\bfseries{\requiprefix}\stepcounter{requicount}\therequicount\normalfont.~\bfseries
}
%
% From https://tex.stackexchange.com/questions/1230/reference-name-of-description-list-item-in-latex
\makeatletter
\def\namedlabel#1{\begingroup
	\def\@currentlabel{\requiprefix\therequicount}%
	\phantomsection\label{#1}\endgroup
}
\makeatother
%
% Usage example:
% \begin{requidescr} % CUSTOM from CDC, with love
%   \item[\namedlabel{req:xaxis} Cluster on Y axis] Something more about that here.
% \end{requidescr}
% I especially like \ref{req:xaxis}.

==> addon/macros-math.tex <==
% Multi-set

\RequirePackage{xparse}
\NewDocumentCommand{\MultiS}{m o}{%
  \IfValueTF{#2}{%
    \ensuremath{\mathfrak{M}#1\left|#2\right|}%
  }{%else
    \ensuremath{\mathfrak{M}#1}%
  }%
}


==> addon/memorandum-for-authors.tex <==
% !TeX root = ../main.tex
%
\section*{For us authors: some tips and tricks}
\label{sec:memo}
%%%
%%% Start of: preliminary commands to be used exclusively in this file.
%%%
\newglossaryentry{test}{name={test},description={A fictionary test}}
\newacronym{testacro}{TA}{Test Acronym}
%%%
%%% End of: preliminary commands to be used exclusively in this file.
%%%
%
% --------------------------------
% About comments
% --------------------------------
%
\hl{For your comments}, please use the
\todo[inline]{\texttt{todo} environment, either in-line or }
or aside.
\todo{aside}
%
You can even add missing figures with the \verb|\missingfigure| command (see \cref{fig:example:missing:figure}).
\begin{figure}[b]
\missingfigure{\texttt{{\textbackslash}missingfigure} command}
\caption{A missing figure}
\label{fig:example:missing:figure}
\end{figure}
%
\\
%
% --------------------------------
% About inline lists
% --------------------------------
%
\hl{For lowercase-roman-enumerated inline lists}, please use
\begin{iiilist}
\item the
\item \texttt{iiilist}
\item environment.
\end{iiilist}
It is a custom command you find in \verb|addons/commands.tex|. It is based on the \verb|\inparaenum| command, from package \textit{paralist}.
%
\\
%
% --------------------------------
% About keywords
% --------------------------------
%
\hl{For specific terms}, which may change in the future, add a \hl{glossary} entry in \texttt{addons/glossary.tex},
and use
\begin{iiilist}
\item the \texttt{gls} command to use them (e.g., \gls{test}),
\item the \texttt{Gls} command for capitalising them (e.g., \Gls{test}),
\item the \texttt{glspl} command for obtaining their plural form (e.g., \glspl{test}), and
\item the \texttt{Glspl} command for for obtaining their plural capitalised form (e.g., \Glspl{test}).
\end{iiilist}
It turns out to be very useful in those situations in which the co-authors do not remember, for example, whether they should indicate the sequences of executed actions as ``traces'' or ``runs''. To solve the issue and avoid that all co-authors write different things, they can decide on a temporary solution (say, ``traces''), make it a glossary entry (say, \verb+\newglossaryentry{actx}{name={trace},description={...}}+), use \verb+\gls{actx}+ (or similar commands -- see above) every time they want to say that thing, and when the opinion on the best term will change (in favour of ``runs''), it will be enough to change the glossary entry definition (\verb+\newglossaryentry{actxeq}{name={run},description={...}}+) and see it varied everywhere it was used in the text. Another use case is: ``AB Testing'' or ``AB testing''? To avoid that the ``T''s of ``testing'' occur as upper-case sometimes, and as lower-case at times, a single glossary entry comes handy!
%
\\
%
\hl{For acronyms}, they are meant be defined within the same file as follows: \texttt{{\textbackslash}newacronym\{testacro\}\{TA\}\{Test Acronym\}}.
They can be referenced by using \texttt{{\textbackslash}Gls} (plus variants for plural forms etc.).
Result is, you get the full version the first time the acronym is used
-- \texttt{{\textbackslash}gls\{testacro\}} is displayed as \Gls{testacro}.
From the second time onwards, the call will return the acronym only, without any description:
\texttt{{\textbackslash}gls\{testacro\}} is displayed as \Gls{testacro}.
To force the representation to have either long or short versions, use
\texttt{{\textbackslash}acrlong\{testacro\}}
(leading to \acrlong{testacro})
or
\texttt{{\textbackslash}acrshort\{testacro\}}
(displaying \acrshort{testacro}).
Acronyms are collected in \texttt{addons/glossary.tex} too.
%
\\
%
\hl{To refer to sections, tables, figures, etc.}, please use the \texttt{cref} command (e.g., \cref{sec:memo}).
\texttt{Cref} capitalises and expands the specifier of the referred document part (e.g., \Cref{fig:example:missing:figure}). It is best to be used at the beginning of phrases, whereas \texttt{cref} uses the abbreviation (e.g., \cref{fig:example:missing:figure}).

\begin{AuthNote}[CDC][Anything to add?]
	We can also add author's notes with the \verb|\begin{AuthNote}...\end{AuthNote}| environment. The optional parameters can be passed to the environment to add (1) your name tag or any in-line title, and (2) a side-note-like title.
\end{AuthNote}

==> addon/reduce-subsubsection-margin.tex <==
% https://tex.stackexchange.com/a/105577
%% Save the class definition of \subparagraph
\let\llncssubparagraph\subparagraph
%% Provide a definition to \subparagraph to keep titlesec happy
\let\subparagraph\paragraph
%% Load titlesec
\usepackage{titlesec}
%% Revert \subparagraph to the llncs definition
\let\subparagraph\llncssubparagraph
\titlespacing{\subsubsection}{0pt}{*0.5}{*0.5}


==> addon/squeeze.tex <==
%% Saving trees -- put this in the preamble
\usepackage{newtxtext}
%% Do not let the Times package affect the monospaced font (Courier is utterly ugly)
\renewcommand{\ttdefault}{cmtt}
%% Shrinking white space here and there…
\usepackage[subtle]{savetrees}
%\addtolength{\topmargin}{-1\baselineskip} % Careful!
%\addtolength{\textheight}{2\baselineskip} % Careful!
%% save space around floats (tables, algo's, fig's):
\setlength{\textfloatsep}{8pt}% Reduce \textfloatsep
%% save more space by suppressing vertical space between paragraphs
% \parskip1pt
%% To remove the starting indentation in footnotes.
% \deffootnote{0.5em}{0em}{\textsuperscript{\thefootnotemark}\,}

==> figures/AltResp-ChnResp--x-automaton.tex <==
\def\taskASymbol{\taskr}
\def\taskBSymbol{\taskv}
\def\taskCSymbol{\taskp}
\def\taskDSymbol{\Task{\$}}
%
\begin{tikzpicture}[->, >=stealth', shorten >=1pt, auto, bend angle=45, initial text = {}]
  \tikzstyle{every state}=[minimum size=1em, align=center]

  \node[state, initial, accepting]    (0) {$\AuSt_0$};
  \node[state, above right=of 0]      (1) {$\AuSt_1$};
  \node[state, below right=of 0]      (2) {$\AuSt_2$};
  \node[state, right=of 2]            (3) {$\AuSt_3$};
  \node[state, above=of 3, fill=gray] (4) {$\AuSt_4$};
  \path
  (0) edge [loop above] node [above left]  {$\AuSym \in \bar{\AuAlph} \cup \{\taskp, \taskv\}$}    (0)
  (0) edge []           node [above]       {$\taskDSymbol$}                                        (1)
  (1) edge [bend left]  node [above]       {$\taskCSymbol$}                                        (0)
  (0) edge []           node [above]       {$\taskASymbol$}                                        (2)
  (2) edge [bend left]  node [above]       {$\taskBSymbol$}                                        (0)
  (2) edge [loop below] node [below]       {$\AuSym \in \bar{\AuAlph} \cup \{\taskCSymbol\}$}      (2)
  (2) edge []           node [above]       {$\taskDSymbol$}                                        (3)
  (3) edge [bend left]  node [above]       {$\taskCSymbol$}                                        (2)
  (1) edge []           node [above right] {$\AuSym \in \AuAlph \setminus \{\taskCSymbol\}$}       (4)
  (2) edge []           node [left]        {$\taskASymbol$}                                        (4)
  (3) edge []           node [right]       {$\AuSym \in \AuAlph \setminus \{\taskCSymbol\}$}       (4)
  (4) edge [loop right] node [right]       {$\AuSym \in \AuAlph$}                                  (4)
  ;  
\end{tikzpicture}

==> figures/AltResp-ChnResp-Prec--x-automaton.tex <==
%
\begin{tikzpicture}[->, >=stealth', shorten >=1pt, auto, bend angle=45, initial text = {}]
  \tikzstyle{every state}=[minimum size=1em, align=center]

  \node[state, initial, accepting]          (0) {$\AuSt_0$};
  \node[state, above right=of 0]            (1) {$\AuSt_1$};
  \node[state, below right=of 0, accepting] (2) {$\AuSt_2$};
  \node[state, left=of 2]                   (3) {$\AuSt_3$};
  \node[state, right=of 2]                  (4) {$\AuSt_4$};
  \node[state, above right=of 4]            (5) {$\AuSt_5$};
  \node[state, right=of 5]                  (6) {$\AuSt_6$};
  \node[state, right=of 1]                  (7) {$\AuSt_7$};
  \node[state, above right=of 5, fill=gray]       (X) {$\AuSt_8$};
  \node[left=of 3]                         (X3) {\textcolor{gray}{to $\AuSt_8$}};
  \node[right=of 4]                        (X4) {\textcolor{gray}{to $\AuSt_8$}};
  \path
  (0) edge [loop above] node [above left]  {$\AuSym \in \bar{\AuAlph}' \cup \{\taskp,\taskv\}$}                                      (0)
  (0) edge []           node [above]  {$\taskr$}                                                         (1)
  (0) edge []           node [above]  {$\taske$}                                                         (X3)
  (1) edge [bend left]  node [above]  {$\taskv$}                                                         (0)
  (1) edge []           node [below]  {$\tasku$}                                                         (5)
  (1) edge [bend left]  node [below]  {$\Task{\$}$}                                                      (7)
  (1) edge [loop left]  node [left]   {$\AuSym \in \bar{\AuAlph}' \cup \{\taskp\}$}                      (1)
  (1) edge [bend left]  node [above]  {$\taske,\taskr$}                                                  (X)
  (7) edge []           node [below]  {$\taskp$}                                                         (1)
  (7) edge []           node [above]  {$\AuSym \in \AuAlph \setminus\{\taskp\}$}                         (X)
  (0) edge []           node [above]  {$\tasku$}                                                         (2)
  (2) edge [loop below] node [below]  {$\AuSym \in \bar{\AuAlph}' \cup \{\tasku,\taskv,\taske,\taskp\}$} (2)
  (2) edge []           node [above]  {$\Task{\$}$}                                                      (4)
  (2) edge [bend left]  node [above]  {$\taskr$}                                                         (5)
  (5) edge []           node [above]  {$\taskv$}                                                         (2)
  (5) edge [bend left]  node [below]  {$\Task{\$}$}                                                      (6)
  (5) edge [loop below] node [below]  {$\AuSym \in \bar{\AuAlph}' \cup \{\tasku,\taske,\taskp\}$}        (5)
  (5) edge []           node [above]  {$\taskr$}                                                         (X)
  (6) edge []           node [below]  {$\taskp$}                                                         (5)
  (6) edge [bend right] node [right]  {$\AuSym \in \AuAlph \setminus\{\taskp\}$}                         (X)
  (0) edge [bend right] node [right]  {$\Task{\$}$}                                                      (3)
  (3) edge []           node [right]   {$\taskp$}                                                        (0)
  (3) edge [bend left]  node [below]  {$\AuSym \in \AuAlph \setminus \{\taskp\}$}                        (X3)
  (4) edge [bend left]  node [above]  {$\taskp$}                                                         (2)
  (4) edge [bend right] node [below]  {$\AuSym \in \AuAlph \setminus \{\taskp\}$}                        (X4)
  (X) edge [loop right] node [right]  {$\AuSym \in \AuAlph$}                                             (X)
  ;  
\end{tikzpicture}

==> figures/AltResp-ChnResp-Prec-AtMoOne--x-automaton.tex <==
%
\begin{tikzpicture}[->, >=stealth', shorten >=1pt, auto, bend angle=45, initial text = {}]
  \tikzstyle{every state}=[minimum size=1em,align=center]

  \node[state, initial, accepting]          (0) {$\AuSt_0$};
  \node[state, below left=of 0]             (2) {$\AuSt_2$};
  \node[state, above right=of 0, accepting] (5) {$\AuSt_5$};
  \node[state, above=of 5]                  (6) {$\AuSt_6$};
  \node[state, above=of 4]                  (7) {$\AuSt_7$};
  \node[state, right=of 7, accepting]       (8) {$\AuSt_8$};
  \node[state, below=of 8, accepting]       (4) {$\AuSt_4$};
  \node[state, right=of 6]                  (9) {$\AuSt_9$};
  \node[state, above right=of 8]            (10) {$\AuSt_{10}$};
  \node[state, below right=of 4]            (11) {$\AuSt_{11}$};
  \node[state, left=of 11]                  (3) {$\AuSt_3$};
  \node[state, above left=of 3]             (1) {$\AuSt_1$};
  \node[left=of 6]                          (X6) {\textcolor{gray}{to $\AuSt_{12}$}};
  \node[right=of 2]                         (X2) {\textcolor{gray}{to $\AuSt_{12}$}};
  \node[below left=of 1]                    (X3) {\textcolor{gray}{to $\AuSt_{12}$}};
  \node[below=of 5]                         (X7) {\textcolor{gray}{to $\AuSt_{12}$}};
  \node[below=of 10]                        (X4) {\textcolor{gray}{to $\AuSt_{12}$}};
  \node[above=of 10]                        (X9) {\textcolor{gray}{to $\AuSt_{12}$}};
  \node[state, right=of 10, fill=gray]      (X) {$\AuSt_{12}$};
  \path
  (0) edge [loop above]  node [above] {$\AuSym\!\!\in\!\! \bar{\AuAlph}' \cup \{\taskv\}$} (0)
  (0) edge []            node [below] {$\taskdollar$}        (1)
  (0) edge []            node [above] {$\taskr$}             (2)
  (0) edge []            node [above] {$\taske$}             (X7)
  (0) edge []            node [right] {$\tasku$}             (5)
  (0) edge []            node [below] {$\taskp$}             (4)
  (1) edge []            node [below] {$\AuSym\!\!\in\!\! \AuAlph\!\setminus\!\!\{\taskp\}$} (X2)
  (1) edge []            node [below] {$\taskp$}             (4)
  (2) edge [bend right]  node [above] {$\taskv$}             (0)
  (2) edge [loop left]   node [left]  {$\AuSym\!\!\in\!\!\bar{\AuAlph}'$} (2)
  (2.south) edge [bend right] node [above]  {$\taskdollar$}  (3)
  (2) edge [bend left]   node [left]  {$\tasku$}             (6)
  (2.south) edge [bend right] node [below left]  {$\taskp$}  (11)
  (2) edge []            node [below right]  {${\taskr,\taske}$} (X2)
  (3) edge []            node [above] {$\taskp$}             (11)
  (3) edge []            node [above] {$\taskp$}             (11)
  (3) edge []            node [above] {$\AuSym\!\!\in\!\! \AuAlph\!\setminus\!\!\{\taskp\}$} (X3)
  (4) edge [loop below]  node [left]  {$\sigma\!\!\in\!\!\bar{\AuAlph}' \cup \{\taskv\}$} (4)
  (4) edge [bend right]  node [right] {$\tasku$}             (8)
  (4) edge [bend left]   node [right] {$\taskr$}             (11)
  (4) edge [bend right]  node [right] {$\taske,\taskp,\taskdollar$} (X4)
  (5) edge [loop right]  node [right] {$\AuSym\!\!\in\!\! \bar{\AuAlph}' \cup \{\taske,\tasku,\taskv\}$} (5)
  (5) edge []            node [right] {$\taskr$}             (6)
  (5) edge []            node [below] {$\taskdollar$}        (7)
  (5) edge []            node [above] {$\taskp$}             (8)
  (6) edge [loop above]  node [left]  {$\AuSym\!\!\in\!\! \bar{\AuAlph}' \cup \{\taske,\tasku\}$} (6)
  (6) edge [bend right]  node [left]  {$\taskv$}             (5)
  (6) edge []            node [above] {$\taskr$}             (X6)
  (6) edge []            node [above] {$\taskdollar$}        (9)
  (6) edge []            node [below] {$\taskp$}             (10)
  (7) edge []            node [below] {$\taskp$}             (8)
  (7) edge []            node [above left]  {$\AuSym\!\!\in\!\! \AuAlph \setminus\!\! \{\taskp\}$} (X7)
  (8) edge [loop below]  node [left]  {$\AuSym\!\!\in\!\!\bar{\AuAlph}' \cup \{\taske,\tasku,\taskv\}$} (8)
  (8) edge []            node [above] {$\taskr$} (10)
  (8) edge []            node [above] {$\taskp,\taskdollar$} (X4)
  (9) edge []            node [above] {$\taskp$}             (10)
  (9) edge []            node [above] {$\AuSym\!\!\in\!\! \AuAlph\!\setminus\!\!\{\taskp\}$} (X9)
  (10) edge [bend right] node [above] {$\taskv$}             (8)
  (10) edge [loop above] node [above] {$\AuSym\!\!\in\!\! \bar{\AuAlph}' \cup \{\taske,\tasku\}$} (8)
  (10) edge []           node [below] {$\taskp,\taskr,\taskdollar$} (X)
  (11) edge []           node [left]  {$\taskv$}            (4)
  (11) edge [bend right] node [right] {$\tasku$}            (10)
  (11) edge [loop below] node [right] {$\AuSym\!\!\in\!\! \bar{\AuAlph}'$} (11)
  (11) edge [bend right] node [right] {$\taske,\taskp, \taskr,\taskdollar$} (X)
  ;  
\end{tikzpicture}

==> figures/absorbing-automaton.tex <==
\begin{tikzpicture}[->, >=stealth', shorten >=1pt, auto, bend angle=45, initial text = {}]
  \tikzstyle{every state}=[minimum size=1em, align=center]

  \node[state, initial, fill=gray] (0) {$\AuSt_0$};

  \path
  (0) edge [loop above] node []        {$\AuSym \in \AuAlph$} (0)
  ;  
\end{tikzpicture}

==> figures/declare-tikz/absence.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center)]\node[DECLARE.task,DECLARE.existcon=$0..m$]{\paramx};\end{tikzpicture}

==> figures/declare-tikz/altprec.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=8*\DTZU]
 \node[DECLARE.task,] (1) {$\paramx$};
 \node[DECLARE.task,right of=1] (2) {$\paramy$};
   
 \path (1) edge [DECLARE.alt.prec] node {} (2);
\end{tikzpicture}

==> figures/declare-tikz/altresp.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=8*\DTZU]
 \node[DECLARE.task,] (1) {$\paramx$};
 \node[DECLARE.task,right of=1] (2) {$\paramy$};
   
 \path (1) edge [DECLARE.alt.resp] node {} (2);
\end{tikzpicture}

==> figures/declare-tikz/altsucc.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=8*\DTZU]
 \node[DECLARE.task,] (1) {$\paramx$};
 \node[DECLARE.task,right of=1] (2) {$\paramy$};
   
 \path (1) edge [DECLARE.alt.succ] node {} (2);
\end{tikzpicture}

==> figures/declare-tikz/atmostone.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center)]\node[DECLARE.task,DECLARE.existcon=$0..1$]{\paramx};\end{tikzpicture}

==> figures/declare-tikz/chnprec.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=8*\DTZU]
 \node[DECLARE.task,] (1) {$\paramx$};
 \node[DECLARE.task,right of=1] (2) {$\paramy$};
   
 \path (1) edge [DECLARE.chn.prec] node {} (2);
\end{tikzpicture}

==> figures/declare-tikz/chnresp.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=8*\DTZU]
 \node[DECLARE.task,] (1) {$\paramx$};
 \node[DECLARE.task,right of=1] (2) {$\paramy$};
   
 \path (1) edge [DECLARE.chn.resp] node {} (2);
\end{tikzpicture}

==> figures/declare-tikz/chnsucc.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=8*\DTZU]
 \node[DECLARE.task,] (1) {$\paramx$};
 \node[DECLARE.task,right of=1] (2) {$\paramy$};
   
 \path (1) edge [DECLARE.chn.succ] node {} (2);
\end{tikzpicture}

==> figures/declare-tikz/coex.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=8*\DTZU]
 \node[DECLARE.task,] (1) {$\paramx$};
 \node[DECLARE.task,right of=1] (2) {$\paramy$};
   
 \path (1) edge [DECLARE.coex] node {} (2);
\end{tikzpicture}

==> figures/declare-tikz/end.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center)]\node[DECLARE.task,DECLARE.existcon=End]{\paramx};\end{tikzpicture}

==> figures/declare-tikz/existence.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center)]\node[DECLARE.task,DECLARE.existcon=$n..\ast$]{\paramx};\end{tikzpicture}

==> figures/declare-tikz/init.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center)]\node[DECLARE.task,DECLARE.existcon=Init]{\paramx};\end{tikzpicture}

==> figures/declare-tikz/notchnsucc.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=8*\DTZU]
 \node[DECLARE.task,] (1) {$\paramx$};
 \node[DECLARE.task,right of=1] (2) {$\paramy$};
   
 \path (1) edge [DECLARE.chn.succ,DECLARE.neg] node {} (2);
\end{tikzpicture}

==> figures/declare-tikz/notcoex.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=8*\DTZU]
 \node[DECLARE.task,] (1) {$\paramx$};
 \node[DECLARE.task,right of=1] (2) {$\paramy$};
   
 \path (1) edge [DECLARE.coex,DECLARE.neg] node {} (2);
\end{tikzpicture}

==> figures/declare-tikz/notsucc.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=8*\DTZU]
 \node[DECLARE.task,] (1) {$\paramx$};
 \node[DECLARE.task,right of=1] (2) {$\paramy$};
   
 \path (1) edge [DECLARE.succ,DECLARE.neg] node {} (2);
\end{tikzpicture}

==> figures/declare-tikz/participation.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center)]\node[DECLARE.task,DECLARE.existcon=$1..\ast$]{\paramx};\end{tikzpicture}

==> figures/declare-tikz/prec.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=8*\DTZU]
 \node[DECLARE.task,] (1) {$\paramx$};
 \node[DECLARE.task,right of=1] (2) {$\paramy$};
   
 \path (1) edge [DECLARE.prec] node {} (2);
\end{tikzpicture}

==> figures/declare-tikz/resex.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=8*\DTZU]
 \node[DECLARE.task,] (1) {$\paramx$};
 \node[DECLARE.task,right of=1] (2) {$\paramy$};
   
 \path (1) edge [DECLARE.resex] node {} (2);
\end{tikzpicture}

==> figures/declare-tikz/resp.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=8*\DTZU]
 \node[DECLARE.task,] (1) {$\paramx$};
 \node[DECLARE.task,right of=1] (2) {$\paramy$};
   
 \path (1) edge [DECLARE.resp] node {} (2);
\end{tikzpicture}

==> figures/declare-tikz/succ.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=8*\DTZU]
 \node[DECLARE.task,] (1) {$\paramx$};
 \node[DECLARE.task,right of=1] (2) {$\paramy$};
   
 \path (1) edge [DECLARE.succ] node {} (2);
\end{tikzpicture}

==> figures/figure-declare-map.tex <==
% !TeX program = lualatex
% !BIB program = biber
% !TeX spellcheck = en_UK
% !TeX encoding = utf8
%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3*\DTZU and 5*\DTZU,DECLARE.task/.append style={inner sep=10,minimum width=10em,minimum height=10ex}]
% \node[DECLARE.task] (payselection) {Pay for \\ selection reg. \\ (p)};
 \node[DECLARE.task,DECLARE.existcon={$0..1$ \\ Init}]            (createaccount) {Create \\ candidate account \\ (c)};
 \node[DECLARE.task,right=of createaccount]                       (register) {Register for \\ selection round \\ (r)};
 \node[DECLARE.task,below=of register]                            (uploadscore) {Upload \\ admission test score \\ (t)};
 \node[DECLARE.task,right=of register]                            (entereval) {Enter \\ evaluation phase \\ (v)};
 \node[DECLARE.task,below=of entereval]                           (rejection) {Receive \\ rejection notification \\ (n)};
 \node[DECLARE.task,right=of rejection]                           (admission) {Receive \\ admission notification \\ (y)};
 \node[DECLARE.task,right=of admission]                           (pay) {Pay \\ subscription fee \\ (\$)};
 \node[DECLARE.task,above=of pay,DECLARE.existcon={$0..1$}]       (preenrol) {Pre-enrol \\ in the program \\ (p)};
 \node[DECLARE.task,right=of pay]                                 (uploaddoc) {Upload \\ certificates \\ (u)};
 \node[DECLARE.task,above=of uploaddoc,DECLARE.existcon={$0..1$}] (enrol) {Enrol \\ in the program \\ (e)};

 \path (uploadscore) edge [DECLARE.prec] node {} (entereval);
 \draw (createaccount) [DECLARE.prec] -- (register);
 \draw (register) [DECLARE.alt.succ] -- (entereval);
 \draw (entereval) [DECLARE.alt.prec] -- (rejection);
 \draw (entereval) [DECLARE.alt.prec] -| (admission);
 \draw (admission) [DECLARE.neg,DECLARE.succ] -- (rejection);
 \draw (admission) [DECLARE.prec] -- (preenrol);
 \draw ([xshift = +2.0\DTZU]pay.north) [DECLARE.chn.resp] -- ([xshift = +2.0\DTZU]preenrol.south);
 \draw ([xshift = -2.0\DTZU]pay.north) [DECLARE.prec] -- ([xshift = -2.0\DTZU]preenrol.south);
 \draw (preenrol) [DECLARE.prec] -- (enrol);
 \draw (uploaddoc) [DECLARE.prec] -- (enrol);
 
% \path (applycast) edge [DECLARE.succ] node {} (removecast);
% \path (performxray) edge [DECLARE.prec] node {} (applycast);
% \path (performsurgery) edge [DECLARE.resp] node {} (prescriberehab);
% \draw (performxray.north) [DECLARE.prec] |- (performreposition.west);
% \draw (performxray.south) [DECLARE.prec] |- (performsurgery.west);
\end{tikzpicture}	

==> figures/identity-automaton.tex <==
\begin{tikzpicture}[->, >=stealth', shorten >=1pt, auto, bend angle=45, initial text = {}]
  \tikzstyle{every state}=[minimum size=1em, align=center]

  \node[state, initial, accepting] (0) {$\AuSt_0$};

  \path
  (0) edge [loop above] node []    {$\AuSym \in \AuAlph$} (0)
  ;  
\end{tikzpicture}

==> sections/declare-lang-example.tex <==
% !TeX program = pdflatex
% !BIB program = bibtex
% !TeX spellcheck = en_UK
% !TeX encoding = utf8
% !TeX root = ../main.tex
%
\begin{example}[A {\Declare} process specification]\label{ex:declare:spec}
%\begin{sloppypar}
%
%
%
\Cref{fig:declare:map:uni} portrays an example of declarative specification for the admission process of an international Bachelor's program.
This example considers the {\Declare} repertoire of templates.
The process begins with the creation of an account in the university portal (henceforth, \taskc). To specify that {\taskc} is the initial task, we write \Ini{\taskc}, graphically depicted with the {\IniTmp} label in the tag on top of the activity box.
{\IniTmp} is a unary template and \Ini{\taskc} assigns its variable with activity \taskc.
Unary templates in {\Declare} are also known as \emph{existence} templates.
We indicate that not more than one account can be created per process run with \AtMo{\taskc}.
In the diagram, it is indicated with the $0..1$ label in the tag.

To register for a selection round (\taskr), an account must have been created before \Prec{\taskc}{\taskr}. We express this rule with \Prec{\taskc}{\taskr}, which is a shorthand notation for $\left(\Prec{x_1}{x_2},\left\{(x_1,\taskc),(x_2,\taskr)\right\}\right)$.
{\PrecTmp} is a binary template and \Prec{\taskc}{\taskr}, graphically depicted as
\begin{scriptsize}
	\begin{tikzpicture}[baseline]
	\node[DECLARE.task,anchor=base] (1) {\taskc};
	\node[DECLARE.task,right=of 1] (2) {\taskr};
	
	\path (1) edge [DECLARE.prec] node {} (2);
	\end{tikzpicture}%
\end{scriptsize}%
, assigns {\taskc} and {\taskr} to its first and second variable, respectively.
Binary templates in {\Declare} are commonly named as \emph{relation} templates.

Every registration to a selection round (\taskr) gives access to a uniquely corresponding evaluation phase (\taskv).
After \taskr, {\taskv} eventually follows and no other registrations are allowed until {\taskv} completes. We write \AltRes{\taskr}{\taskv}, graphically depicted as
\begin{scriptsize}
	\begin{tikzpicture}[baseline]
	\node[DECLARE.task,anchor=base] (1) {\taskr};
	\node[DECLARE.task,right=of 1] (2) {\taskv};
	
	\path (1) edge [DECLARE.alt.resp] node {} (2);
	\end{tikzpicture}%
\end{scriptsize}%
.
The evaluation requires {\taskr} to be completed before and {\taskv} will not recur unless a new registration is issued: \AltPrec{\taskr}{\taskv},
\begin{scriptsize}
	\begin{tikzpicture}[baseline]
	\node[DECLARE.task,anchor=base] (1) {\taskr};
	\node[DECLARE.task,right=of 1] (2) {\taskv};
	
	\path (1) edge [DECLARE.alt.prec] node {} (2);
	\end{tikzpicture}%
\end{scriptsize}%
.
Typically, if both \AltRes{\taskr}{\taskv} and \AltPrec{\taskr}{\taskv} hold true, we compactly represent them jointly with the \emph{mutual} relation constraint \AltSucc{\taskr}{\taskv}
\begin{scriptsize}
	\begin{tikzpicture}[baseline]
	\node[DECLARE.task,anchor=base] (1) {\taskr};
	\node[DECLARE.task,right=of 1] (2) {\taskv};
	
	\path (1) edge [DECLARE.alt.succ] node {} (2);
	\end{tikzpicture}%
\end{scriptsize}%
.
%
An admission test score has to be uploaded in the platform to access the evaluation phase: \Prec{\taskt}{\taskv}.
Evaluation phases are necessary for the committee to return rejections (\taskn) and notifications of admission (\tasky), thus \AltPrec{\taskv}{\tasky} and \AltPrec{\taskv}{\taskn} hold.

After the admission has been notified, the candidate will not receive a rejection any longer -- \NotResp{\tasky}{\taskn}, drawn in \cref{fig:declare:map:uni} as 
\begin{scriptsize}
	\begin{tikzpicture}[baseline]
	\node[DECLARE.task,anchor=base] (1) {\tasky};
	\node[DECLARE.task,right=of 1] (2) {\taskn};
	
	\path (1) edge [DECLARE.neg,DECLARE.succ] node {} (2);
	\end{tikzpicture}%
\end{scriptsize}%
.
\NotResp{\tasky}{\taskn} falls under the category of the \emph{negative} relation constraints, as the occurrence of {\tasky} \emph{disables} {\taskn} in the remainder of the process execution.

Only if candidates receive a notification of admission, they will be entitled to pre-enrol in the program (\Prec{\tasky}{\taskp}). The candidates are considered as pre-enrolled immediately after they pay the subscription fee (\ChnResp{\taskdollar}{\taskp}, shown as follows in the diagram:
\begin{scriptsize}
	\begin{tikzpicture}[baseline]
	\node[DECLARE.task,anchor=base] (1) {\taskdollar};
	\node[DECLARE.task,right=of 1] (2) {\taskp};
	
	\path (1) edge [DECLARE.chn.resp] node {} (2);
	\end{tikzpicture}%
\end{scriptsize}%
).
Also, candidates cannot be considered as pre-enrolled if they have not paid the subscription fee: 
\Prec{\taskdollar}{\taskp}.
Not more than one pre-enrolment is allowed per candidate: \AtMo{\taskp}.
To enrol in the program (\taske), the candidate must have pre-enrolled -- \Prec{\taskp}{\taske} -- and uploaded the necessary school and language certificates -- \Prec{\tasku}{\taske}.
%
%
%
%
%\end{sloppypar}
%

\begin{figure}[tb]
	\centering
	\resizebox{\columnwidth}{!}{\input{figures/figure-declare-map}}
	\caption{The {\Declare} map of the admission process at a university.}
	\label{fig:declare:map:uni}
\end{figure}
\end{example}

==> sections/modelling.tex <==
\todo[inline]{Warning: the full text is taken as-is from \cite{DiCiccio.Montali/PMH2022:DeclarativeProcessMining}. The formal definition should be changed because it does not cater for branching. See \cite{DiCiccio.etal/IS2016:EfficientDiscoveryTarget} for a definition we gave (though not full-fledged; we should make it more rigorous).}

Formally, we define a declarative process specification as follows.
\begin{definition}[Declarative process specification]\label{def:decspec}
	A \emph{declarative process specification} is a tuple $\DecSpec=(\DecRepertoire,\ProActvts,\CnsSet)$ where
	\begin{compactitem}[$\bullet$]
		\item $\DecRepertoire$ is a finite non-empty set of \emph{templates}, where each template is a predicate $\DecTemp(x_1, \ldots, x_m) \in \DecRepertoire$ on variables $x_1, \ldots, x_m$ (with $m \in \mathbb{N}$ the \emph{arity} of $\DecTemp$),	
		\item $\ProActvts$ is a finite non-empty set of %(names of) 
			\emph{activities},
		\item $\CnsSet$ is a finite set of \emph{constraints}, namely pairs $(\DecTemp(x_1, \ldots, x_m),\kappa)$ where $\DecTemp(x_1, \ldots, x_m)$ is a template from  $\DecRepertoire$, and $\kappa$ is a mapping that, for every $i \in \{1,\ldots,m\}$ assigns variable $x_i$ with a set of activities $\kappa(x_i) = a_i \in \ProActvts$;
% $m$ whose variables are assigned by a mapping with activities $x_i \stackrel{\kappa}{\mapsto} a_i$ with $a_i \in \ProActvts$, $1 \leqslant i \leqslant m$. % associating templates to sets of activities, where every constraint $c = (\DclrSty{r}, \{a_1, \ldots, a_n\})$ assigns an activity $a_i$ ($0 \leqslant i \leqslant n$, where $n$ is the arity of $\DclrSty{r}$) to a variable of $\DclrSty{r}$. 
		we compactly denote such a constraint with $\DclrSty{k}(a_1, \ldots, a_m)$.
		%	\item {$\Pi(A)$ is a set of constraints defined over the activities,}
		%	\item {$\S(\pi),\,\pi\in\Pi$ is a function assigning semantics to a constraint, and}
		%	\item {$\Phi= \prod_{\pi\in\Pi}\S(\pi)$ is the model comprised of the product of constraints, given that the language used to express the constraints is closed for common properties such as concatenation, intersection, Kleene star, and so on, as is the case for automata-based languages such as regular expressions and \Gls{ltl}.}
	\end{compactitem}
\end{definition}
%
%\subsubsection{An example of declarative process specification}
% Giovanni: questa la levo perché non credo che ci serva 
%\label{sec:declare:example}
%#\input{sections/declare-lang-example}

%\bigskip
%The semantics of most declarative process specification languages and \Declare in particular can be expressed with \gls{ltlf}. In the next section, we introduce the basic notions of the language and explain how declarative constraints relate to it.
So far, we have been attaching an informal semantics to {\Declare} and its templates. In the next section, we provide a more systematic and formal characterization. 

==> snippet/side-by-side-figure-and-table_snippet.tex <==
\begin{figure}[tb]
\CenterFloatBoxes
\begin{floatrow}
  \ttabbox{%
  % % %
  % % % TABLE
  % % %
    \begin{tabular}{  c  c  c  c  }
      \toprule
      Col1 & Col2 & Col3 & Col4 \\
      \midrule
       & & & \\
      \midrule
       & & & \\
       & & & \\
       & & & \\
       & & & \\
      \bottomrule
    \end{tabular} %
  }{%
    \caption{A table} %
    \label{table:table} %
  }
  \killfloatstyle
  \ffigbox{%
  % % %
  % % % FIGURE
  % % %
    \includegraphics[width=0.45\textwidth]{} %
  }{%
    \caption{A figure} %
    \label{fig:figure} %
  }
\end{floatrow}
\end{figure}



==> tables/table-DECLARE-constraints-as-LTLf-rcon.tex <==
%!TEX root = ../main.tex
%
%\renewcommand{\arraystretch}{1.6}
\begin{tabular}{ l p{4.2cm} l}
	\toprule
	\textbf{Constraint} & 
	\textbf{\acrshort{ltlf} expression~\cite{DeGiacomo.Vardi/IJCAI2013:LDLf}} &
	\textbf{\acrshort{rf}~\cite{Cecconi.etal/ICPM2020:TLBasedMeasurementProcessMining}}
\\

%	\midrule
%	\multicolumn{3}{l}{Existence constraints}\\

\midrule
$ \AtLe{\taska} $&%\equiv \textit{Existence}(1, \taska)$ &
$ \ltlevtly \taska $ &
$ \lstart \limply \ltlevtly \taska$ 
\\

$\Init{\taska}$ &
$ \taska $ &
$ \lstart \limply \taska $
\\

$\End{\taska}$ &
$ \ltlalws \ltlevtly \taska $ &
$ \lend \limply \taska $ 
\\

$\Uniq{\taska}$ &
$ \ltlalws (\taska \rightarrow \ltlnext(\lnot \ltlevtly \taska)) $ &
$ \taska \limply \ltlnext(\lnot \ltlevtly \taska) $ 
\\

%	\midrule
%	\multicolumn{3}{l}{Relation constraints}\\

%\midrule
$\ResEx{\taska}{\taskb}$ &
$ \ltlevtly \taska \rightarrow \ltlevtly \taskb $ &
$ \taska \limply (\ltlevtly \taskb \vee \ltlonce \taskb)$
\\

$\Resp{\taska}{\taskb}$ &
$ \ltlalws(\taska \rightarrow \ltlevtly \taskb ) $ &
$ \taska \limply \ltlevtly \taskb$
\\

$\AltResp{\taska}{\taskb}$ &
$ \ltlalws(\taska \rightarrow \ltlevtly \taskb ) \wedge \ltlalws(\taska \rightarrow \ltlnext(\lnot\taska \ltlwntil \taskb)) $ &
$ \taska \limply \ltlnext(\lnot\taska \ltluntil \taskb) $ 
\\

$\ChaResp{\taska}{\taskb}$ &
$ \ltlalws(\taska \rightarrow \ltlevtly \taskb ) \wedge \ltlalws(\taska \rightarrow\ltlnext \taskb) $ &
$ \taska \limply \ltlnext \taskb $
\\

$\Prec{\taska}{\taskb}$ &
$ \lnot\taskb \ltlwntil \taska $ &
$ \taskb \limply \ltlonce \taska $
\\

$\AltPrec{\taska}{\taskb}$ &
$ (\lnot\taskb \ltlwntil \taska) \wedge \ltlalws(\taskb \rightarrow \ltlnext  (\lnot\taskb \ltlwntil \taska))$ &
$ \taskb \limply \ltlyday(\lnot\taskb \ltlsince \taska) $
\\

$\ChaPrec{\taska}{\taskb}$ &
$ (\lnot\taskb \ltlwntil \taska) \wedge \ltlalws(\ltlnext \taskb \rightarrow \taska) $ &
$ \taskb \limply \ltlyday \taska $
\\

$ \Succ{\taska}{\taskb} $ &
$ \ltlalws(\taska \rightarrow \ltlevtly \taskb ) \wedge (\lnot\taskb \ltlwntil \taska)$&
$ (\taska \vee \taskb) \limply (\taska \wedge \ltlevtly \taskb)\vee(\taskb \wedge \ltlonce \taska) $
\\

$ \AltSucc{\taska}{\taskb} $ &
\makecell[l]{
	$ 
	\ltlalws(\taska \rightarrow \ltlevtly \taskb ) \wedge \ltlalws(\taska \rightarrow \ltlnext(\lnot\taska \ltlwntil \taskb)) 
	$ \\
	$\wedge (\lnot\taskb \ltlwntil \taska) \wedge \ltlalws(\taskb \rightarrow \ltlnext  (\lnot\taskb \ltlwntil \taska)) $} 
&
\makecell[l]{
	$ (\taska \vee \taskb) \limply            (\taska \wedge \ltlnext(\lnot\taska \ltluntil \taskb))\vee$\\
	\phantom{$(\taska \vee \taskb) \limply$}$ (\taskb \wedge \ltlyday(\lnot\taskb \ltlsince \taska)) $
}
\\

$ \ChaSucc{\taska}{\taskb} $&
\makecell[l]{
	$ \ltlalws(\taska \rightarrow \ltlevtly \taskb ) \wedge \ltlalws(\taska \rightarrow\ltlnext \taskb) $\\
	$ \wedge (\lnot\taskb \ltlwntil \taska) \wedge \ltlalws(\ltlnext \taskb \rightarrow \taska) $
}
&
$ (\taska \vee \taskb) \limply (\taska \wedge \ltlnext \taskb) \vee (\taskb \wedge \ltlyday \taska)$
\\

$ \CoExi{\taska}{\taskb}  $ &
$ (\ltlevtly\taska \wedge\ltlevtly\taskb) \vee (\lnot\ltlevtly\taska \wedge\lnot\ltlevtly\taskb )$&
\makecell[l]{
	$ (\taska \vee \taskb) \limply            (\taska\wedge\ltlevtly\taskb)\vee(\taska\wedge\ltlonce\taskb)\vee$\\
	\phantom{$(\taska \vee \taskb) \limply$}$ (\taskb\wedge\ltlevtly\taska)\vee(\taskb\wedge\ltlonce\taska) $
}
\\

$ \NotCoExi{\taska}{\taskb} $ &
$ \ltlalws(\taska \rightarrow \lnot\ltlevtly \taskb ) \wedge \ltlalws(\taskb \rightarrow \lnot\ltlevtly \taska )$&
\makecell[l]{
	$ (\taska \vee \taskb) \limply            (\taska\wedge \lnot\ltlonce\taskb \wedge \lnot\ltlevtly\taskb)\vee$\\
	\phantom{$(\taska \vee \taskb) \limply$}$ (\taskb\wedge \lnot\ltlonce\taska \wedge \lnot\ltlevtly\taska)$	
}
\\

\bottomrule
\end{tabular}

==> tables/table-DECLARE-constraints-def-examples-gfx.tex <==
%!TEX root = ../main.tex
\renewcommand{\arraystretch}{1.6}
%\begin{tabular}{ l p{3cm} >{{\goodexample}~}l >{{\goodexample}~}l >{{\badexample}~}l c c}
\begin{tabular}{ l p{28mm} l l l l c}
	\toprule
	\textbf{Constraint} & 
	\textbf{Explanation} & 
	\multicolumn{4}{c}{\textbf{Examples}} & 
	\textbf{Notation} \\  % bcaaccbbbaba
	
	\midrule
	\multicolumn{7}{l}{Existence constraints}\\
	
	\midrule
	
%	$\Exi{n}{\taska}$ & % [^$2]*($2[^$2]*){$1,}[^$2]*
%	Activity $\taska$ occurs at least $n$ times in the trace &
%	\multicolumn{4}{l}{~} &
%	\DrawExistence[\qquad\taska\qquad]
%	\\

	
	$\Ini{\taska}$ &
	{\taska} is the \emph{first} to occur & 
  \GoodExampleMark $\tup{\taska,\taskc,\taskc}$ & \GoodExampleMark $\tup{\taska,\taskb,\taska,\taskc}$ & \BadExampleMark $\tup{\taskc,\taskc}$ & \BadExampleMark $\tup{\taskb,\taska,\taskc}$ & \DrawInit[\qquad\taska\qquad]\\

	$\AtLe{\taska}$ & % \equiv \Exi{1}{\taska}$ &
	$\taska$ occurs at least \emph{once} &
	\GoodExampleMark  $\tup{\taskb,\taskc,\taska,\taskc}$  &  
	\GoodExampleMark  $\tup{\taskb,\taskc,\taska,\taska,\taskc}$ &
	\BadExampleMark  $\tup{\taskb,\taskc,\taskc}$  & 
	\BadExampleMark  $\tup{\taskc}$ &
	\DrawParticipation[\qquad\taska\qquad]
	\\
	
%	$\Abse{m+1}{\taska}$ & % [^$2]*($2[^$2]*){0,$max}[^$2]*
%	$\taska$ occurs at most $m$ times &
%	\multicolumn{4}{l}{~} &
%	\DrawAbsence[\qquad\taska\qquad]
%	\\
	
	$\AtMo{\taska}$ & % \equiv \Abse{2}{\taska}$ &
	$\taska$ occurs at most \emph{once} &
	\GoodExampleMark $\tup{\taskb,\taskc,\taskc}$ & \GoodExampleMark $\tup{\taskb,\taskc,\taska,\taskc}$ &
	\BadExampleMark $\tup{\taskb,\taskc,\taska,\taska,\taskc}$ & \BadExampleMark $\tup{\taskb,\taskc,\taska,\taskc,\taska,\taska}$ &
	\DrawAtmostone[\qquad\taska\qquad]
	\\

	
	$\End{\taska}$ &
	{\taska} is the \emph{last} to occur &
	\GoodExampleMark $\tup{\taskb,\taskc,\taska}$ & \GoodExampleMark $\tup{\taskb,\taska,\taskc,\taska}$ &
	\BadExampleMark $\tup{\taskb,\taskc}$ & \BadExampleMark $\tup{\taskb,\taska,\taskc}$ &
	\DrawEnd[\qquad\taska\qquad]
	\\
	
	\midrule
	\multicolumn{7}{l}{Relation constraints}\\
	\midrule
	$\ResEx{\taska}{\taskb}$ &
	If {\taska} occurs in the trace, then {\taskb} occurs as well &
	\GoodExampleMark $\tup{\taskb,\taskc,\taska,\taska,\taskc}$ & \GoodExampleMark $\tup{\taskb,\taskc,\taskc}$ &
	\BadExampleMark $\tup{\taskc,\taska,\taska,\taskc}$ & \BadExampleMark $\tup{\taska,\taskc,\taskc}$ &
	\DrawResex[\taska][\taskb]
	\\
	$\Resp{\taska}{\taskb}$ &
	If {\taska} occurs, then {\taskb} occurs after {\taska} &
	\GoodExampleMark $\tup{\taskc,\taska,\taska,\taskc,\taskb}$ & \GoodExampleMark $\tup{\taskb,\taskc,\taskc}$ &
	\BadExampleMark $\tup{\taskc,\taska,\taska,\taskc}$ & \BadExampleMark $\tup{\taskb,\taska,\taskc,\taskc}$ &
	\DrawResp[\taska][\taskb]
	\\
	$\AltResp{\taska}{\taskb}$ &
	Each time {\taska} occurs, then {\taskb} occurs afterwards, and no other {\taska} recurs in between &
	\GoodExampleMark $\tup{\taskc,\taska,\taskc,\taskb}$ & \GoodExampleMark $\tup{\taska,\taskb,\taskc,\taska,\taskc,\taskb}$ &
	\BadExampleMark $\tup{\taskc,\taska,\taska,\taskc,\taskb}$ & \BadExampleMark $\tup{\taskb,\taska,\taskc,\taska,\taskc,\taskb}$ &
	\DrawAltresp[\taska][\taskb]
	\\
	$\ChnResp{\taska}{\taskb}$ &
	Each time {\taska} occurs, then {\taskb} occurs immediately afterwards &
	\GoodExampleMark $\tup{\taskc,\taska,\taskb,\taskb}$ & \GoodExampleMark $\tup{\taska,\taskb,\taskc,\taska,\taskb}$ &
	\BadExampleMark $\tup{\taskc,\taska,\taskc,\taskb}$ & \BadExampleMark $\tup{\taskb,\taskc,\taska}$ &
	\DrawChnresp[\taska][\taskb]
	\\
	$\Prec{\taska}{\taskb}$ &
	{\taskb} occurs only if preceded by {\taska} &
	\GoodExampleMark $\tup{\taskc,\taska,\taskc,\taskb,\taskb}$ & \GoodExampleMark $\tup{\taska,\taskc,\taskc}$ &
	\BadExampleMark $\tup{\taskc,\taskc,\taskb,\taskb}$ & \BadExampleMark $\tup{\taskb,\taska,\taskc,\taskc}$ &
	\DrawPrec[\taska][\taskb]
	\\
	$\AltPrec{\taska}{\taskb}$ &
	Each time {\taskb} occurs, it is preceded by {\taska} and no other {\taskb} can recur in between &
	\GoodExampleMark $\tup{\taskc,\taska,\taskc,\taskb,\taska}$ & \GoodExampleMark $\tup{\taska,\taskb,\taskc,\taska,\taska,\taskc,\taskb}$ &
	\BadExampleMark $\tup{\taskc,\taska,\taskc,\taskb,\taskb,\taska}$ & \BadExampleMark $\tup{\taska,\taskb,\taskb,\taska,\taskb,\taskc,\taskb}$ &
	\DrawAltprec[\taska][\taskb]
	\\
	$\ChnPrec{\taska}{\taskb}$ &
	Each time {\taskb} occurs, then {\taska} occurs immediately beforehand &
	\GoodExampleMark $\tup{\taska,\taskb,\taskc,\taska}$ & \GoodExampleMark $\tup{\taska,\taskb,\taska,\taska,\taskb,\taskc}$ &
	\BadExampleMark $\tup{\taskb,\taskc,\taska}$ & \BadExampleMark $\tup{\taskb,\taska,\taska,\taskc,\taskb}$ &
	\DrawChnprec[\taska][\taskb]
	\\
	\midrule
	\multicolumn{7}{l}{Mutual relation constraints}\\
	\midrule
	$\CoExi{\taska}{\taskb}$ &
	If {\taskb} occurs, then {\taska} occurs, and vice versa &
	\GoodExampleMark $\tup{\taskc,\taska,\taskc,\taskb,\taskb}$ & \GoodExampleMark $\tup{\taskb,\taskc,\taskc,\taska}$ &
	\BadExampleMark $\tup{\taskc,\taska,\taskc}$ & \BadExampleMark $\tup{\taskb,\taskc,\taskc}$ &
	\DrawCoex[\taska][\taskb]
	\\
	$\Succ{\taska}{\taskb}$ &
	{\taska} occurs if and only if it is followed by {\taskb} &
	\GoodExampleMark $\tup{\taskc,\taska,\taskc,\taskb,\taskb}$ & \GoodExampleMark $\tup{\taska,\taskc,\taskc,\taskb}$ &
	\BadExampleMark $\tup{\taskb,\taska,\taskc}$ & \BadExampleMark $\tup{\taskb,\taskc,\taskc,\taska}$ &
	\DrawSucc[\taska][\taskb]
	\\
	$\AltSucc{\taska}{\taskb}$ &
	{\taska} and {\taskb} if and only if the latter follows the former, and they alternate each other in the trace &
	\GoodExampleMark $\tup{\taskc,\taska,\taskc,\taskb,\taska,\taskb}$ & \GoodExampleMark $\tup{\taska,\taskb,\taskc,\taska,\taskb,\taskc}$ &
	\BadExampleMark $\tup{\taskc,\taska,\taska,\taskc,\taskb,\taskb}$ & \BadExampleMark $\tup{\taskb,\taska,\taskc}$ &
	\DrawAltsucc[\taska][\taskb]
	\\
	$\ChnSucc{\taska}{\taskb}$ &
	{\taska} and {\taskb} occur if and only if the latter immediately follows the former &
	\GoodExampleMark $\tup{\taskc,\taska,\taskb,\taska,\taskb}$ & \GoodExampleMark $\tup{\taskc,\taskc,\taskc}$ &
	\BadExampleMark $\tup{\taskc,\taska,\taskc,\taskb}$ & \BadExampleMark $\tup{\taskc,\taskb,\taska,\taskc}$ &
	\DrawChnsucc[\taska][\taskb]
	\\
	\midrule
	\multicolumn{7}{l}{Negative relation constraints}\\
	\midrule
	$\NotCoExi{\taska}{\taskb}$ &
	{\taska} and {\taskb} never occur together &
	\GoodExampleMark $\tup{\taskc,\taskc,\taskc,\taskb,\taskb,\taskb}$ & \GoodExampleMark $\tup{\taskc,\taskc,\taska,\taskc}$ &
	\BadExampleMark $\tup{\taska,\taskc,\taskc,\taskb,\taskb}$ & \BadExampleMark $\tup{\taskb,\taskc,\taska,\taskc}$ &
	\DrawNotcoex[\taska][\taskb]
	\\
	$\NotSucc{\taska}{\taskb}$ &
	{\taskb} cannot occur after {\taska} &
	\GoodExampleMark $\tup{\taskb,\taskb,\taskc,\taska,\taska}$ & \GoodExampleMark $\tup{\taskc,\taskb,\taskb,\taskc,\taska}$ &
	\BadExampleMark $\tup{\taska,\taska,\taskc,\taskb,\taskb}$ & \BadExampleMark $\tup{\taska,\taskb,\taskb}$ &
	\DrawNotsucc[\taska][\taskb]
	\\
	$\NotChnSucc{\taska}{\taskb}$ &
	{\taska} and {\taskb} cannot occur contiguously &
	\GoodExampleMark $\tup{\taska,\taskc,\taskb,\taska,\taskc,\taskb}$ & \GoodExampleMark $\tup{\taskb,\taskb,\taska,\taska}$ &
	\BadExampleMark $\tup{\taska,\taskb,\taskc,\taska,\taskb}$ & \BadExampleMark $\tup{\taskc,\taska,\taskb,\taskc}$ &
	\DrawNotchnsucc[\taska][\taskb]
	\\
	\bottomrule
\end{tabular}

==> tables/table-DECLARE-constraints-def-examples.tex <==
%!TEX root = ../main.tex
\renewcommand{\arraystretch}{1.6}
%\begin{tabular}{ l p{3cm} >{{\goodexample}~}l >{{\goodexample}~}l >{{\badexample}~}l c c}
\begin{tabular}{ l p{5cm} l l l l }
	\toprule
	\textbf{Constraint} & 
	\textbf{Explanation} & 
	\multicolumn{4}{c}{\textbf{Examples}}
	\\
	\midrule
	\multicolumn{6}{l}{Existence constraints}\\
	
	\midrule
	$\Exi{n}{\taska}$ & % [^$2]*($2[^$2]*){$1,}[^$2]*
	Activity $\taska$ occurs at least $n$ times &
	\multicolumn{4}{l}{~}
	\\
	
	$\AtLe{\taska} \equiv \Exi{1}{\taska}$ &
	$\taska$ occurs at least \emph{once} &
	\GoodExampleMark $ \Task{bcac} $  &  
	\GoodExampleMark $ \Task{bcaac} $  &
	\BadExampleMark $ \Task{bcc} $ & 
	\BadExampleMark $ \taskc $
	\\
	
	$\Abse{m+1}{\taska}$ & % [^$2]*($2[^$2]*){0,$max}[^$2]*
	$\taska$ occurs at most $m$ times &
	\multicolumn{4}{l}{~}
	\\
	
	$\AtMo{\taska} \equiv \Abse{2}{\taska}$ &
	$\taska$ occurs at most \emph{once} &
	\GoodExampleMark \Task{bcc} & \GoodExampleMark \Task{bcac} &
	\BadExampleMark \Task{bcaac} & \BadExampleMark \Task{bcacaa}
	\\
	
	$\Ini{\taska}$ &
	{\taska} is the \emph{first} to occur &
	\GoodExampleMark \Task{acc} & \GoodExampleMark \Task{abac} &
	\BadExampleMark \Task{cc} & \BadExampleMark \Task{bac}
	\\
	
	$\End{\taska}$ &
	{\taska} is the \emph{last} to occur &
	\GoodExampleMark \Task{bca} & \GoodExampleMark \Task{baca} &
	\BadExampleMark \Task{bc} & \BadExampleMark \Task{bac}
	\\
	
	\midrule
	\multicolumn{6}{l}{Relation constraints}\\
	\midrule
	$\ResEx{\taska}{\taskb}$ &
	If {\taska} occurs, then {\taskb} occurs as well &
	\GoodExampleMark \Task{bcaac} & \GoodExampleMark \Task{bcc} &
	\BadExampleMark \Task{caac} & \BadExampleMark \Task{acc}
	\\
	$\Resp{\taska}{\taskb}$ &
	If {\taska} occurs, then {\taskb} occurs after {\taska} &
	\GoodExampleMark \Task{caacb} & \GoodExampleMark \Task{bcc} &
	\BadExampleMark \Task{caac} & \BadExampleMark \Task{bacc}
	\\
	$\AltResp{\taska}{\taskb}$ &
	Each time {\taska} occurs, then {\taskb} occurs afterwards, and no other {\taska} recurs in between &
	\GoodExampleMark \Task{cacb} & \GoodExampleMark \Task{abcacb} &
	\BadExampleMark \Task{caacb} & \BadExampleMark \Task{bacacb}
	\\
	$\ChnResp{\taska}{\taskb}$ &
	Each time {\taska} occurs, then {\taskb} occurs immediately afterwards &
	\GoodExampleMark \Task{cabb} & \GoodExampleMark \Task{abcab} &
	\BadExampleMark \Task{cacb} & \BadExampleMark \Task{bca}
	\\
	$\Prec{\taska}{\taskb}$ &
	{\taskb} occurs only if preceded by {\taska} &
	\GoodExampleMark \Task{cacbb} & \GoodExampleMark \Task{acc} &
	\BadExampleMark \Task{ccbb} & \BadExampleMark \Task{bacc}
	\\
	$\AltPrec{\taska}{\taskb}$ &
	Each time {\taskb} occurs, it is preceded by {\taska} and no other {\taskb} recurs in between &
	\GoodExampleMark \Task{cacba} & \GoodExampleMark \Task{abcaacb} &
	\BadExampleMark \Task{cacbba} & \BadExampleMark \Task{abbabcb}
	\\
	$\ChnPrec{\taska}{\taskb}$ &
	Each time {\taskb} occurs, then {\taska} occurs immediately beforehand &
	\GoodExampleMark \Task{abca} & \GoodExampleMark \Task{abaabc} &
	\BadExampleMark \Task{bca} & \BadExampleMark \Task{baacb}
	\\
	\midrule
	\multicolumn{6}{l}{Mutual relation constraints}\\
	\midrule
	$\CoExi{\taska}{\taskb}$ &
	If {\taskb} occurs, then {\taska} occurs, and vice versa &
	\GoodExampleMark \Task{cacbb} & \GoodExampleMark \Task{bcca} &
	\BadExampleMark \Task{cac} & \BadExampleMark \Task{bcc}
	\\
	$\Succ{\taska}{\taskb}$ &
	{\taska} occurs if and only if it is followed by {\taskb} &
	\GoodExampleMark \Task{cacbb} & \GoodExampleMark \Task{accb} &
	\BadExampleMark \Task{bac} & \BadExampleMark \Task{bcca}
	\\
	$\AltSucc{\taska}{\taskb}$ &
	{\taska} and {\taskb} if and only if the latter follows the former, and they alternate each other &
	\GoodExampleMark \Task{cacbab} & \GoodExampleMark \Task{abcabc} &
	\BadExampleMark \Task{caacbb} & \BadExampleMark \Task{bac}
	\\
	$\ChnSucc{\taska}{\taskb}$ &
	{\taska} and {\taskb} occur if and only if the latter immediately follows the former &
	\GoodExampleMark \Task{cabab} & \GoodExampleMark \Task{ccc} &
	\BadExampleMark \Task{cacb} & \BadExampleMark \Task{cbac}
	\\
	\midrule
	\multicolumn{6}{l}{Negative relation constraints}\\
	\midrule
	$\NotCoExi{\taska}{\taskb}$ &
	{\taska} and {\taskb} never occur together &
	\GoodExampleMark \Task{cccbbb} & \GoodExampleMark \Task{ccac} &
	\BadExampleMark \Task{accbb} & \BadExampleMark \Task{bcac}
	\\
	$\NotSucc{\taska}{\taskb}$ &
	{\taska} never occurs before {\taskb} &
	\GoodExampleMark \Task{bbcaa} & \GoodExampleMark \Task{cbbca} &
	\BadExampleMark \Task{aacbb} & \BadExampleMark \Task{abb}
	\\
	$\NotChnSucc{\taska}{\taskb}$ &
	{\taska} and {\taskb} occur if and only if the latter does not immediately follows the former &
	\GoodExampleMark \Task{acbacb} & \GoodExampleMark \Task{bbaa} &
	\BadExampleMark \Task{abcab} & \BadExampleMark \Task{cabc}
	\\
	\bottomrule
\end{tabular}

==> tables/table-DECLARE-constraints-def-formula.tex <==
%!TEX root = ../main.tex
\renewcommand{\arraystretch}{1.6}
%\begin{tabular}{ l p{3cm} >{{\goodexample}~}l >{{\goodexample}~}l >{{\badexample}~}l c c}
\begin{tabular}{ l l p{4cm}} % { l p{3cm} l l l l c}
	\toprule
		\textbf{Constraint} & 
		\textbf{{\ltlpf} formulation} &
		\textbf{Explanation} % & 
%		\multicolumn{4}{c}{\textbf{Examples}} & 
		\\
	\midrule
		\multicolumn{3}{l}{Existence constraints}\\ % \multicolumn{7}{l}{Existence constraints}\\
	
	\midrule
		$\Exi{n}{\taska}$ &
		$ \LTLfut ( \taska \land \underbrace{ \LTLfut ( \LTLnext \taska \land \ldots \land \LTLfut ( \LTLnext \taska ) ) }_{n-1} ) $ &
		Activity $\taska$ occurs at least $n$ times in the trace % &
		%\multicolumn{4}{l}{~} &
		%\DrawExistence[\taska]
		\\
		
		$\Part{\taska} \equiv \Exi{1}{\taska}$ &
		$ \LTLfut \taska $ & 
		$\taska$ occurs at least \emph{once} % &
%		\GoodExampleMark $ \taskize{bcac} $  &  
%		\GoodExampleMark $ \taskize{bcaac} $  &
%		\BadExampleMark $ \taskize{bcc} $ & 
%		\BadExampleMark $ \taskc $ &
		\\
		$\Abse{m+1}{\taska}$ & % [^$2]*($2[^$2]*){0,$max}[^$2]*
		$ \LTLalwFut ( \lnot \taska \lor \underbrace{\LTLalwFut ( \LTLnext \lnot \taska \lor \ldots \lor \LTLalwFut ( \LTLnext \lnot \taska ) ) }_{m} ) $ &
		$\taska$ occurs at most $m$ times % &
		%\multicolumn{4}{l}{~} &
		%\DrawAbsence[\taska]
		\\
		$\Uniq{\taska} \equiv \Abse{2}{\taska}$ &
		$ \LTLalwFut ( \lnot \taska \lor \LTLalwFut ( \LTLnext \lnot \taska ) ) $ &
		$\taska$ occurs at most \emph{once} % &
%		\GoodExampleMark \taskize{bcc} & \GoodExampleMark \taskize{bcac} &
%		\BadExampleMark \taskize{bcaac} & \BadExampleMark \taskize{bcacaa} &
		\\

		$\Ini{\taska}$ &
		$ \taska $ &
		{\taska} is the \emph{first} to occur % &
%		\GoodExampleMark \taskize{acc} & \GoodExampleMark \taskize{abac} &
%		\BadExampleMark \taskize{cc} & \BadExampleMark \taskize{bac} &
		\\

		$\End{\taska}$ &
		$ \LTLalwFut \LTLfut \taska $ &
		{\taska} is the \emph{last} to occur % &
%		\GoodExampleMark \taskize{bca} & \GoodExampleMark \taskize{baca} &
%		\BadExampleMark \taskize{bc} & \BadExampleMark \taskize{bac} &
		\\
		
	\midrule
	\multicolumn{3}{l}{Relation constraints}\\ %\multicolumn{7}{l}{Relation constraints}\\
	\midrule
	$\ResEx{\taska}{\taskb}$ &
	$ \LTLfut \taska \limplies \LTLfut \taskb $ &
	If {\taska} occurs in the trace, then {\taskb} occurs as well % &
%	\GoodExampleMark \taskize{bcaac} & \GoodExampleMark \taskize{bcc} &
%	\BadExampleMark \taskize{caac} & \BadExampleMark \taskize{acc} &
	\\
	$\Resp{\taska}{\taskb}$ &
	$ \LTLalwFut(\taska \limplies \LTLfut \taskb ) $ &
	If {\taska} occurs, then {\taskb} occurs after {\taska} % &
%	\GoodExampleMark \taskize{caacb} & \GoodExampleMark \taskize{bcc} &
%	\BadExampleMark \taskize{caac} & \BadExampleMark \taskize{bacc} &
	\\
	$\AltResp{\taska}{\taskb}$ &
	$ \LTLalwFut(\taska \limplies \LTLnext (\lnot \taska \LTLuntil \taskb) ) $ &
	Each time {\taska} occurs, then {\taskb} occurs afterwards, and no other {\taska} recurs in between % &
%	\GoodExampleMark \taskize{cacb} & \GoodExampleMark \taskize{abcacb} &
%	\BadExampleMark \taskize{caacb} & \BadExampleMark \taskize{bacacb} &
	\\
	$\ChaResp{\taska}{\taskb}$ &
	$ \LTLalwFut(\taska \limplies \LTLnext \taskb) $ &
	Each time {\taska} occurs, then {\taskb} occurs immediately afterwards % &
%	\GoodExampleMark \taskize{cabb} & \GoodExampleMark \taskize{abcab} &
%	\BadExampleMark \taskize{cacb} & \BadExampleMark \taskize{bca} &
	\\
	$\Prec{\taska}{\taskb}$ &
	$ \LTLalwFut(\taska \limplies \LTLpast \taskb) $ &
	{\taskb} occurs only if preceded by {\taska} % &
%	\GoodExampleMark \taskize{cacbb} & \GoodExampleMark \taskize{acc} &
%	\BadExampleMark \taskize{ccbb} & \BadExampleMark \taskize{bacc} &
	\\
	$\AltPrec{\taska}{\taskb}$ &
	$ \LTLalwFut(\taska \limplies \LTLprev (\lnot \taskb \LTLsince \taska ) ) $ &
	Each time {\taskb} occurs, it is preceded by {\taska} and no other {\taskb} can recur in between % &
%	\GoodExampleMark \taskize{cacba} & \GoodExampleMark \taskize{abcaacb} &
%	\BadExampleMark \taskize{cacbba} & \BadExampleMark \taskize{abbabcb} &
	\\
	$\ChaPrec{\taska}{\taskb}$ &
	$ \LTLalwFut(\taska \limplies \LTLprev \taskb) $ &
	Each time {\taskb} occurs, then {\taska} occurs immediately beforehand % &
%	\GoodExampleMark \taskize{abca} & \GoodExampleMark \taskize{abaabc} &
%	\BadExampleMark \taskize{bca} & \BadExampleMark \taskize{baacb} &
	\\
	\midrule
	\multicolumn{3}{l}{Mutual relation constraints}\\ % \multicolumn{7}{l}{Mutual relation constraints}\\
	\midrule
	$\CoExi{\taska}{\taskb}$ &
	$ \LTLfut \taska \lcoimplies \LTLfut \taskb  $ &
	If {\taskb} occurs, then {\taska} occurs, and vice versa % &
%	\GoodExampleMark \taskize{cacbb} & \GoodExampleMark \taskize{bcca} &
%	\BadExampleMark \taskize{cac} & \BadExampleMark \taskize{bcc} &
	\\
	$\Succ{\taska}{\taskb}$ &
	$ \LTLalwFut( ( \taska \limplies \LTLfut \taskb ) \land ( \taskb \limplies \LTLpast \taska ) ) $ &
	{\taska} occurs if and only if followed by {\taskb} % &
%	\GoodExampleMark \taskize{cacbb} & \GoodExampleMark \taskize{accb} &
%	\BadExampleMark \taskize{bac} & \BadExampleMark \taskize{bcca} &
	\\
	$\AltSucc{\taska}{\taskb}$ &
	$ \LTLalwFut( (\taska \limplies \LTLnext (\lnot \taska \LTLuntil \taskb) ) \land (\taskb \limplies \LTLprev (\lnot \taska \LTLsince \taskb ) ) ) $ &
	{\taska} and {\taskb} if and only if the latter follows the former, and they alternate each other in the trace % &
%	\GoodExampleMark \taskize{cacbab} & \GoodExampleMark \taskize{abcabc} &
%	\BadExampleMark \taskize{caacbb} & \BadExampleMark \taskize{bac} &
	\\
	$\ChaSucc{\taska}{\taskb}$ &
	$ \LTLalwFut( (\taska \limplies \LTLnext \taskb) \land (\taskb \limplies \LTLprev \taska) ) $ &
	{\taska} and {\taskb} occur if and only if the latter immediately follows the former % &
%	\GoodExampleMark \taskize{cabab} & \GoodExampleMark \taskize{ccc} &
%	\BadExampleMark \taskize{cacb} & \BadExampleMark \taskize{cbac} &
	\\
	\midrule
	\multicolumn{3}{l}{Negative relation constraints}\\ % \multicolumn{7}{l}{Negative relation constraints}\\
	\midrule
	$\NotCoExi{\taska}{\taskb}$ &
	$ \LTLalwFut \lnot \taska \lor \LTLalwFut \lnot \taskb $ &
	{\taska} and {\taskb} never occur together % &
%	\GoodExampleMark \taskize{cccbbb} & \GoodExampleMark \taskize{ccac} &
%	\BadExampleMark \taskize{accbb} & \BadExampleMark \taskize{bcac} &
	\\
	$\NotSucc{\taska}{\taskb}$ &
	$ \LTLalwFut ( ( \taska \limplies \LTLalwFut \lnot \taskb ) \land ( \taskb \limplies \LTLalwPast \lnot \taska ) ) $ &
	{\taska} can never occur before {\taskb} % &
%	\GoodExampleMark \taskize{bbcaa} & \GoodExampleMark \taskize{cbbca} &
%	\BadExampleMark \taskize{aacbb} & \BadExampleMark \taskize{abb} &
	\\
	$\NotChaSucc{\taska}{\taskb}$ &
	$ \LTLalwFut ( ( \taska \limplies \LTLnext \lnot \taskb ) \land ( \taskb \limplies \LTLprev \lnot \taska ) ) $ &
	{\taska} and {\taskb} occur if and only if the latter does not immediately follows the former % &
%	\GoodExampleMark \taskize{acbacb} & \GoodExampleMark \taskize{bbaa} &
%	\BadExampleMark \taskize{abcab} & \BadExampleMark \taskize{cabc} &
	\\
	\bottomrule
\end{tabular}

==> tables/table-DECLARE-constraints-def-gfx.tex <==
%!TEX root = ../main.tex
\renewcommand{\arraystretch}{1.6}
%\begin{tabular}{ l p{3cm} >{{\goodexample}~}l >{{\goodexample}~}l >{{\badexample}~}l c c}
\begin{tabular}{ l p{8cm} c}
	\toprule
	\textbf{Constraint} & 
	\textbf{Explanation} & 
	\textbf{Notation} \\  % bcaaccbbbaba
	
	\midrule
	\multicolumn{3}{l}{Existence constraints}\\
	
	\midrule
	$\Exi{n}{\taska}$ & % [^$2]*($2[^$2]*){$1,}[^$2]*
	Activity $\taska$ occurs at least $n$ times in the trace &
	\DrawExistence[\taska]
	\\
	
	$\Part{\taska} \equiv \Exi{1}{\taska}$ &
	$\taska$ occurs at least \emph{once} &
	\DrawParticipation[\taska]
	\\
	
	$\Abse{m+1}{\taska}$ & % [^$2]*($2[^$2]*){0,$max}[^$2]*
	$\taska$ occurs at most $m$ times &
	\DrawAbsence[\taska]
	\\
	
	$\Uniq{\taska} \equiv \Abse{2}{\taska}$ &
	$\taska$ occurs at most \emph{once} &
	\DrawAtmostone[\taska]
	\\
	
	$\Ini{\taska}$ &
	{\taska} is the \emph{first} to occur &
	\DrawInit[\taska]
	\\
	
	$\End{\taska}$ &
	{\taska} is the \emph{last} to occur &
	\DrawEnd[\taska]
	\\
	
	\midrule
	\multicolumn{3}{l}{Relation constraints}\\
	\midrule
	$\ResEx{\taska}{\taskb}$ &
	If {\taska} occurs in the trace, then {\taskb} occurs as well &
	\DrawResex[\taska][\taskb]
	\\
	$\Resp{\taska}{\taskb}$ &
	If {\taska} occurs, then {\taskb} occurs after {\taska} &
	\DrawResp[\taska][\taskb]
	\\
	$\AltResp{\taska}{\taskb}$ &
	Each time {\taska} occurs, then {\taskb} occurs afterwards, and no other {\taska} recurs in between &
	\DrawAltresp[\taska][\taskb]
	\\
	$\ChaResp{\taska}{\taskb}$ &
	Each time {\taska} occurs, then {\taskb} occurs immediately afterwards &
	\DrawChnresp[\taska][\taskb]
	\\
	$\Prec{\taska}{\taskb}$ &
	{\taskb} occurs only if preceded by {\taska} &
	\DrawPrec[\taska][\taskb]
	\\
	$\AltPrec{\taska}{\taskb}$ &
	Each time {\taskb} occurs, it is preceded by {\taska} and no other {\taskb} can recur in between &
	\DrawAltprec[\taska][\taskb]
	\\
	$\ChaPrec{\taska}{\taskb}$ &
	Each time {\taskb} occurs, then {\taska} occurs immediately beforehand &
	\DrawChnprec[\taska][\taskb]
	\\
	\midrule
	\multicolumn{3}{l}{Mutual relation constraints}\\
	\midrule
	$\CoExi{\taska}{\taskb}$ &
	If {\taskb} occurs, then {\taska} occurs, and vice versa &
	\DrawCoex[\taska][\taskb]
	\\
	$\Succ{\taska}{\taskb}$ &
	{\taska} occurs if and only if it is followed by {\taskb} &
	\DrawSucc[\taska][\taskb]
	\\
	$\AltSucc{\taska}{\taskb}$ &
	{\taska} and {\taskb} if and only if the latter follows the former, and they alternate each other in the trace &
	\DrawAltsucc[\taska][\taskb]
	\\
	$\ChaSucc{\taska}{\taskb}$ &
	{\taska} and {\taskb} occur if and only if the latter immediately follows the former &
	\DrawChnsucc[\taska][\taskb]
	\\
	\midrule
	\multicolumn{3}{l}{Negative relation constraints}\\
	\midrule
	$\NotCoExi{\taska}{\taskb}$ &
	{\taska} and {\taskb} never occur together &
	\DrawNotcoex[\taska][\taskb]
	\\
	$\NotSucc{\taska}{\taskb}$ &
	{\taska} can never occur before {\taskb} &
	\DrawNotsucc[\taska][\taskb]
	\\
	$\NotChaSucc{\taska}{\taskb}$ &
	{\taska} and {\taskb} occur if and only if the latter does not immediately follows the former &
	\DrawNotchnsucc[\taska][\taskb]
	\\
	\bottomrule
\end{tabular}

==> tables/table-DECLARE-constraints-formula.tex <==
%!TEX root = ../main.tex
\renewcommand{\arraystretch}{1.6}
%\begin{tabular}{ l p{3cm} >{{\goodexample}~}l >{{\goodexample}~}l >{{\badexample}~}l c c}
\begin{tabular}{ l l p{4cm}} % { l p{3cm} l l l l c}
	\toprule
		\textbf{Constraint} & 
		\textbf{{\ltlpf} formulation} &
%		\textbf{Explanation} % & 
%		\multicolumn{4}{c}{\textbf{Examples}} & 
		\\
	\midrule
		\multicolumn{3}{l}{Existence constraints}\\ % \multicolumn{7}{l}{Existence constraints}\\
	
	\midrule
		$\textit{Existence}(n, \taska)$ &
		$ \LTLfut ( \taska \land \underbrace{ \LTLfut ( \LTLnext \taska \land \ldots \land \LTLfut ( \LTLnext \taska ) ) }_{n-1} ) $ &
%		Activity $\taska$ occurs at least $n$ times in the trace % &
		%\multicolumn{4}{l}{~} &
		%\DrawExistence[\taska]
		\\
		
		$\Part{\taska} \equiv \textit{Existence}(1, \taska)$ &
		$ \LTLfut (\taska) $ & 
%		$\taska$ occurs at least \emph{once} % &
%		\GoodExampleMark $ \taskize{bcac} $  &  
%		\GoodExampleMark $ \taskize{bcaac} $  &
%		\BadExampleMark $ \taskize{bcc} $ & 
%		\BadExampleMark $ \taskc $ &
		\\
		$\textit{Absence}(m+1, \taska)$ & % [^$2]*($2[^$2]*){0,$max}[^$2]*
		$ \LTLalwFut ( \lnot \taska \lor \underbrace{\LTLalwFut ( \LTLnext \lnot \taska \lor \ldots \lor \LTLalwFut ( \LTLnext \lnot \taska ) ) }_{m} ) $ &
%		$\taska$ occurs at most $m$ times % &
		%\multicolumn{4}{l}{~} &
		%\DrawAbsence[\taska]
		\\
		$\Uniq{\taska} \equiv \textit{Absence}(2, \taska)$ &
		$ \LTLalwFut ( \lnot \taska \lor \LTLalwFut ( \LTLnext \lnot \taska ) ) $ &
%		$\taska$ occurs at most \emph{once} % &
%		\GoodExampleMark \taskize{bcc} & \GoodExampleMark \taskize{bcac} &
%		\BadExampleMark \taskize{bcaac} & \BadExampleMark \taskize{bcacaa} &
		\\

		$\Ini{\taska}$ &
		$ \taska $ &
%		{\taska} is the \emph{first} to occur % &
%		\GoodExampleMark \taskize{acc} & \GoodExampleMark \taskize{abac} &
%		\BadExampleMark \taskize{cc} & \BadExampleMark \taskize{bac} &
		\\

		$\End{\taska}$ &
		$ \LTLalwFut \LTLfut ( \taska ) $ &
%		{\taska} is the \emph{last} to occur % &
%		\GoodExampleMark \taskize{bca} & \GoodExampleMark \taskize{baca} &
%		\BadExampleMark \taskize{bc} & \BadExampleMark \taskize{bac} &
		\\
		
	\midrule
	\multicolumn{3}{l}{Relation constraints}\\ %\multicolumn{7}{l}{Relation constraints}\\
	\midrule
	$\ResEx{\paramx}{\paramy}$ &
	$ \LTLfut \paramx \limplies \LTLfut \paramy $ &
	\\
	$\ResEx{\taska}{\taskb}$ &
	$ \LTLfut \taska \limplies \LTLfut \taskb $ &
%	If {\taska} occurs in the trace, then {\taskb} occurs as well % &
%	\GoodExampleMark \taskize{bcaac} & \GoodExampleMark \taskize{bcc} &
%	\BadExampleMark \taskize{caac} & \BadExampleMark \taskize{acc} &
	\\
	$\Resp{\paramx}{\paramy}$ &
	$ \LTLalwFut(\paramx \limplies \LTLfut \paramy ) $ &
	\\
	$\Resp{\taska}{\taskc}$ &
$ \LTLalwFut(\taska \limplies \LTLfut \taskc ) $ &
%	If {\taska} occurs, then {\taskb} occurs after {\taska} % &
%	\GoodExampleMark \taskize{caacb} & \GoodExampleMark \taskize{bcc} &
%	\BadExampleMark \taskize{caac} & \BadExampleMark \taskize{bacc} &
	\\
	$\AltResp{\taska}{\taskb}$ &
	$ \LTLalwFut(\taska \limplies \LTLnext (\lnot \taska \LTLuntil \taskb) ) $ &
%	Each time {\taska} occurs, then {\taskb} occurs afterwards, and no other {\taska} recurs in between % &
%	\GoodExampleMark \taskize{cacb} & \GoodExampleMark \taskize{abcacb} &
%	\BadExampleMark \taskize{caacb} & \BadExampleMark \taskize{bacacb} &
	\\
	$\ChaResp{\taska}{\taskb}$ &
	$ \LTLalwFut(\taska \limplies \LTLnext \taskb) $ &
%	Each time {\taska} occurs, then {\taskb} occurs immediately afterwards % &
%	\GoodExampleMark \taskize{cabb} & \GoodExampleMark \taskize{abcab} &
%	\BadExampleMark \taskize{cacb} & \BadExampleMark \taskize{bca} &
	\\
	$\Prec{\taska}{\taskb}$ &
	$ \LTLalwFut(\taska \limplies \LTLpast \taskb) $ &
%	{\taskb} occurs only if preceded by {\taska} % &
%	\GoodExampleMark \taskize{cacbb} & \GoodExampleMark \taskize{acc} &
%	\BadExampleMark \taskize{ccbb} & \BadExampleMark \taskize{bacc} &
	\\
	$\AltPrec{\taska}{\taskb}$ &
	$ \LTLalwFut(\taska \limplies \LTLprev (\lnot \taskb \LTLsince \taska ) ) $ &
%	Each time {\taskb} occurs, it is preceded by {\taska} and no other {\taskb} can recur in between % &
%	\GoodExampleMark \taskize{cacba} & \GoodExampleMark \taskize{abcaacb} &
%	\BadExampleMark \taskize{cacbba} & \BadExampleMark \taskize{abbabcb} &
	\\
	$\ChaPrec{\taska}{\taskb}$ &
	$ \LTLalwFut(\taska \limplies \LTLprev \taskb) $ &
%	Each time {\taskb} occurs, then {\taska} occurs immediately beforehand % &
%	\GoodExampleMark \taskize{abca} & \GoodExampleMark \taskize{abaabc} &
%	\BadExampleMark \taskize{bca} & \BadExampleMark \taskize{baacb} &
	\\
	\midrule
	\multicolumn{3}{l}{Mutual relation constraints}\\ % \multicolumn{7}{l}{Mutual relation constraints}\\
	\midrule
	$\CoExi{\taska}{\taskb}$ &
	$ \LTLfut \taska \lcoimplies \LTLfut \taskb  $ &
%	If {\taskb} occurs, then {\taska} occurs, and vice versa % &
%	\GoodExampleMark \taskize{cacbb} & \GoodExampleMark \taskize{bcca} &
%	\BadExampleMark \taskize{cac} & \BadExampleMark \taskize{bcc} &
	\\
	$\Succ{\taska}{\taskb}$ &
	$ \LTLalwFut( ( \taska \limplies \LTLfut \taskb ) \land ( \taskb \limplies \LTLpast \taska ) ) $ &
%	{\taska} occurs if and only if followed by {\taskb} % &
%	\GoodExampleMark \taskize{cacbb} & \GoodExampleMark \taskize{accb} &
%	\BadExampleMark \taskize{bac} & \BadExampleMark \taskize{bcca} &
	\\
	$\AltSucc{\taska}{\taskb}$ &
	$ \LTLalwFut( (\taska \limplies \LTLnext (\lnot \taska \LTLuntil \taskb) ) \land (\taskb \limplies \LTLprev (\lnot \taska \LTLsince \taskb ) ) ) $ &
%	{\taska} and {\taskb} if and only if the latter follows the former, and they alternate each other in the trace % &
%	\GoodExampleMark \taskize{cacbab} & \GoodExampleMark \taskize{abcabc} &
%	\BadExampleMark \taskize{caacbb} & \BadExampleMark \taskize{bac} &
	\\
	$\ChaSucc{\taska}{\taskb}$ &
	$ \LTLalwFut( (\taska \limplies \LTLnext \taskb) \land (\taskb \limplies \LTLprev \taska) ) $ &
%	{\taska} and {\taskb} occur if and only if the latter immediately follows the former % &
%	\GoodExampleMark \taskize{cabab} & \GoodExampleMark \taskize{ccc} &
%	\BadExampleMark \taskize{cacb} & \BadExampleMark \taskize{cbac} &
	\\
	\midrule
	\multicolumn{3}{l}{Negative relation constraints}\\ % \multicolumn{7}{l}{Negative relation constraints}\\
	\midrule
	$\NotCoExi{\taska}{\taskb}$ &
	$ \LTLalwFut \lnot \taska \lor \LTLalwFut \lnot \taskb $ &
%	{\taska} and {\taskb} never occur together % &
%	\GoodExampleMark \taskize{cccbbb} & \GoodExampleMark \taskize{ccac} &
%	\BadExampleMark \taskize{accbb} & \BadExampleMark \taskize{bcac} &
	\\
	$\NotSucc{\taska}{\taskb}$ &
	$ \LTLalwFut ( ( \taska \limplies \LTLalwFut \lnot \taskb ) \land ( \taskb \limplies \LTLalwPast \lnot \taska ) ) $ &
%	{\taska} can never occur before {\taskb} % &
%	\GoodExampleMark \taskize{bbcaa} & \GoodExampleMark \taskize{cbbca} &
%	\BadExampleMark \taskize{aacbb} & \BadExampleMark \taskize{abb} &
	\\
	$\NotChaSucc{\taska}{\taskb}$ &
	$ \LTLalwFut ( ( \taska \limplies \LTLnext \lnot \taskb ) \land ( \taskb \limplies \LTLprev \lnot \taska ) ) $ &
%	{\taska} and {\taskb} occur if and only if the latter does not immediately follows the former % &
%	\GoodExampleMark \taskize{acbacb} & \GoodExampleMark \taskize{bbaa} &
%	\BadExampleMark \taskize{abcab} & \BadExampleMark \taskize{cabc} &
	\\
	\bottomrule
\end{tabular}

==> tables/table-DECLARE-templates-formula-activ-target.tex <==
%!TEX root = ../main.tex
\renewcommand{\arraystretch}{1.6}
%\begin{tabular}{ l p{3cm} >{{\goodexample}~}l >{{\goodexample}~}l >{{\badexample}~}l c c}
\begin{tabular}{ l l l l } % { l p{3cm} l l l l c}
	\toprule
	\textbf{Template} & 
	\textbf{{\ltlpf} formulation} &
	\textbf{Activations} & 
	\textbf{Targets} % & 
	%		\multicolumn{4}{c}{\textbf{Examples}} & 
	\\
	\midrule
	\multicolumn{4}{l}{Existence templates}\\ % \multicolumn{7}{l}{Existence templates}\\
	
	\midrule
	$\Exi{n}{\paramx}$ &
	$ \LTLfut ( \paramx \land \underbrace{ \LTLfut ( \LTLnext \paramx \land \ldots \land \LTLfut ( \LTLnext \paramx ) ) }_{n-1} ) $ &
	--
	&
	\paramx
	\\
	
	$\Part{\paramx} \equiv \Exi{1}{\paramx}$ &
	$ \LTLfut \paramx $ &
	--
	&
	\paramx
	\\
	
	$\Abse{m+1}{\paramx}$ & % [^$2]*($2[^$2]*){0,$max}[^$2]*
	$ \LTLalwFut ( \lnot \paramx \lor \underbrace{\LTLalwFut ( \LTLnext \lnot \paramx \lor \ldots \lor \LTLalwFut ( \LTLnext \lnot \paramx ) ) }_{m} ) $ &
	--
	&
	\paramx
	\\
	
	$\Uniq{\paramx} \equiv \Abse{2}{\paramx}$ &
	$ \LTLalwFut ( \lnot \paramx \lor \LTLalwFut ( \LTLnext \lnot \paramx ) ) $&
	--
	&
	\paramx
	\\
	
	$\Ini{\paramx}$ &
	$ \paramx $ &
	--
	&
	\paramx
	\\
	
	$\End{\paramx}$ &
	$ \LTLalwFut \LTLfut \paramx $ &
	--
	&
	\paramx
	\\
	
	\midrule
	\multicolumn{4}{l}{Relation templates}\\ %\multicolumn{7}{l}{Relation templates}\\
	\midrule
	$\ResEx{\paramx}{\paramy}$ &
	$ \LTLfut \paramx \limplies \LTLfut \paramy $ &
	\paramx
	&
	\paramy
	\\
	$\Resp{\paramx}{\paramy}$ &
	$ \LTLalwFut(\paramx \limplies \LTLfut \paramy ) $ &
	\paramx
	&
	\paramy
	\\
	$\AltResp{\paramx}{\paramy}$ &
	$ \LTLalwFut(\paramx \limplies \LTLnext (\lnot \paramx \LTLuntil \paramy) ) $ &
	\paramx
	&
	\paramy
	\\
	$\ChaResp{\paramx}{\paramy}$ &
	$ \LTLalwFut(\paramx \limplies \LTLnext \paramy) $ &
	\paramx
	&
	\paramy
	\\
	% BACKWARD-DIRECTIONAL
	$\Prec{\paramx}{\paramy}$ &
	$ \LTLalwFut(\paramx \limplies \LTLpast \paramy) $ &
	\paramy
	&
	\paramx
	\\
	$\AltPrec{\paramx}{\paramy}$ &
	$ \LTLalwFut(\paramx \limplies \LTLprev (\lnot \paramy \LTLsince \paramx ) ) $ &
	\paramy
	&
	\paramx
	\\
	$\ChaPrec{\paramx}{\paramy}$ &
	$ \LTLalwFut(\paramx \limplies \LTLprev \paramy) $ &
	\paramy
	&
	\paramx
	\\
	\midrule
	\multicolumn{4}{l}{Mutual relation templates}\\ % \multicolumn{7}{l}{Mutual relation templates}\\
	\midrule
	$\CoExi{\paramx}{\paramy}$ &
	$ \LTLfut \paramx \lcoimplies \LTLfut \paramy  $ &
	\paramx, \paramy
	&
	\paramy, \paramx
	\\
	$\Succ{\paramx}{\paramy}$ &
	$ \LTLalwFut( ( \paramx \limplies \LTLfut \paramy ) \land ( \paramy \limplies \LTLpast \paramx ) ) $ &
	\paramx, \paramy
	&
	\paramy, \paramx
	\\
	$\AltSucc{\paramx}{\paramy}$ &
	$ \LTLalwFut( (\paramx \limplies \LTLnext (\lnot \paramx \LTLuntil \paramy) ) \land (\paramy \limplies \LTLprev (\lnot \paramx \LTLsince \paramy ) ) ) $ &
	\paramx, \paramy
	&
	\paramy, \paramx
	\\
	$\ChaSucc{\paramx}{\paramy}$ &
	$ \LTLalwFut( (\paramx \limplies \LTLnext \paramy) \land (\paramy \limplies \LTLprev \paramx) ) $ &
	\paramx, \paramy
	&
	\paramy, \paramx
	\\
	\midrule
	\multicolumn{4}{l}{Negative relation templates}\\ % \multicolumn{7}{l}{Negative relation templates}\\
	\midrule
	$\NotCoExi{\paramx}{\paramy}$ &
	$ \LTLalwFut \lnot \paramx \lor \LTLalwFut \lnot \paramy $ &
	\paramx, \paramy
	&
	\paramy, \paramx
	\\
	$\NotSucc{\paramx}{\paramy}$ &
	$ \LTLalwFut ( ( \paramx \limplies \LTLalwFut \lnot \paramy ) \land ( \paramy \limplies \LTLalwPast \lnot \paramx ) ) $ &
	\paramx, \paramy
	&
	\paramy, \paramx
	\\
	$\NotChaSucc{\paramx}{\paramy}$ &
	$ \LTLalwFut ( ( \paramx \limplies \LTLnext \lnot \paramy ) \land ( \paramy \limplies \LTLprev \lnot \paramx ) ) $ &
	\paramx, \paramy
	&
	\paramy, \paramx
	\\
	\bottomrule
\end{tabular}

==> tables/table-conformance-results.tex <==
\begin{table}[tb]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l S[table-format=1.3] l l}
    	\toprule
    	\textbf{Constraint with trace fitness lower than \num{0.5}}  & \textbf{Tr.\ Fitness} & &
    		\textbf{Constraint with trace fitness \num{0.999} }
    	\\ \cmidrule{1-2}\cmidrule{4-4}
    	\AltPrecShort{\Task{04\_BPT\_005}}{\Task{01\_HOOFD\_030\_2}} & 0.361 & &
    		\AltPrecShort{\Task{01\_HOOFD\_050}}{\Task{01\_HOOFD\_060}} % & 0.999                 
    	\\
    	\AltPrecShort{\Task{01\_HOOFD\_510\_2}}{\Task{END}}          & 0.445 & &                 
    		\AltPrecShort{\{\Task{01\_HOOFD\_030\_1},\Task{04\_BPT\_005}\}}{\Task{01\_HOOFD\_061}} % & 0.999 
    	\\
    	\AltPrecShort{\Task{01\_HOOFD\_515}}{\Task{END}}             & 0.434 & &
    		\AltPrecShort{\Task{01\_HOOFD\_065\_2}}{\Task{01\_HOOFD\_110}} % & 0.999                 
    	\\
    	\AltPrecShort{\Task{01\_BB\_770}}{\Task{END}}                & 0.368 & & 
    		\AltPrecShort{\Task{01\_HOOFD\_180}}{\Task{01\_HOOFD\_195}} % & 0.999                 
    	\\
    	\AltPrecShort{\Task{08\_AWB45\_030}}{\Task{END}}             & 0.164 & &
    		\AltPrecShort{\Task{02\_DRZ\_010}}{\Task{04\_BPT\_005}} % & 0.999 
    	\\ 
    	& & &
    		\AltPrecShort{\{\Task{01\_HOOFD\_030\_1},\Task{01\_HOOFD\_050},\Task{01\_HOOFD\_065\_0}\}}{\Task{02\_DRZ\_010}} % & 0.999                 
    	\\ \bottomrule
    \end{tabular}%
	}
    \caption{BPIC~15\textsubscript{5f} constraints fitness values.}
    \label{tab:fitness}
\end{table}
%

==> tables/table-running-example-discovery-measures.tex <==
\begin{tabular}{@{}lSSSS@{}}
	\toprule
	                              &    \multicolumn{2}{c}{Event-based}     &    \multicolumn{2}{c}{Trace-based}     \\  \cmidrule(r){2-3}\cmidrule(l){4-5}
	\textbf{Constraint}           & \textbf{Confidence} & \textbf{Support} & \textbf{Confidence} & \textbf{Support} \\ \midrule
%	\Ini{\taskc}                  & 1                   & 1                & 1                   & 1                \\
%	\AtMo{\taskc}                 & 1                   & 1                & 1                   & 1                \\
	\Prec{\taskc}{\taskr}         & 1                   & 0.129            & 1                   & 1                \\
	\AltPrec{\taskr}{\taskv}      & 1                   & 0.129            & 1                   & 1                \\
	\AltResp{\taskr}{\taskv}      & 0.997               & 0.129            & 0.996               & 0.996            \\
	\Prec{\taskt}{\taskv}         & 0.997               & 0.129            & 0.996               & 0.996            \\
	\AltPrec{\taskv}{\taskn}      & 1                   & 0.059            & 1                   & 0.461            \\
	\AltPrec{\taskv}{\tasky}      & 1                   & 0.084            & 1                   & 0.856            \\
	\NotResp{\tasky}{\taskn}      & 1                   & 0.084            & 1                   & 0.856            \\
	\Prec{\tasky}{\taskp}         & 1                   & 0.07             & 1                   & 0.715            \\
	\Prec{\taskdollar}{\taskp}    & 1                   & 0.07             & 1                   & 0.715            \\
	\ChnResp{\taskdollar}{\taskp} & 1                   & 0.07             & 1                   & 0.715            \\
	\AtMo{\taskp}                 & 1                   & 1                & 1                   & 1                \\
	\Prec{\taskp}{\taske}         & 1                   & 0.07             & 1                   & 0.715            \\
	\AtMo{\taske}                 & 1                   & 1                & 1                   & 1                \\
	\Prec{\tasku}{\taske}         & 0.985               & 0.069            & 0.985               & 0.704            \\ \bottomrule
\end{tabular}

==> tikzlibraryDECLARE.code.tex <==
%
% This is the DECLARE TikZ library by Claudio Di Ciccio is licensed under a Creative Commons Attribution-ShareAlike 4.0 International License.
% This work is licensed under the Creative Commons Attribution-ShareAlike 4.0 International License. To view a copy of this license, visit http://creativecommons.org/licenses/by-sa/4.0/.
%
% Author: Claudio Di Ciccio
% Website: www.diciccio.net
% Date: 2017/02/08
%
\usetikzlibrary{arrows.meta,decorations.markings}
\def\DTZU {2ex}
\tikzset{
 DECLARE.task/.style={
  rounded corners=1ex,
  minimum width=3em,
  minimum height=1ex,
  align=center,
  font=\sffamily,
  inner sep=5,
  draw
 },
 DECLARE.existcon/.style={
  label={[style={draw,trapezium},yshift=-1\pgflinewidth]above:{\parbox{2em}{\centering \scriptsize \textsc{#1}}}}
 },
 DECLARE.neg/.style={
  semithick,
  postaction={decorate,decoration={markings,
   mark=at position .5 with {\arrow[xshift=0.15*\DTZU]{Bar[width=1.5*\DTZU]}},
   mark=at position .5 with {\arrow[xshift=-0.15*\DTZU]{Bar[width=1.5*\DTZU]}}
  }}
 },
 DECLARE.resex/.style={
  semithick,
  {Circle[length=1*\DTZU,width=1*\DTZU]}-,
  shorten <=-0.5*\DTZU
 },
 DECLARE.resp/.style={
  semithick,rounded corners,
  {Circle[length=1*\DTZU,width=1*\DTZU]}-{Triangle[length=1*\DTZU,width=1*\DTZU]},
  shorten <=-0.5*\DTZU
 },
 DECLARE.alt.resp/.style={
  semithick,rounded corners,
  {Circle[length=1*\DTZU,width=1*\DTZU]}-{Triangle[length=1*\DTZU,width=1*\DTZU]},
  shorten <=-0.5*\DTZU,
  double distance=0.25*\DTZU
 },
 DECLARE.chn.resp/.style={
  semithick,rounded corners,
  preaction={draw, shorten <= -0.5*\DTZU, double distance=0.25*\DTZU, {Circle[length=1*\DTZU,width=1*\DTZU]}-{Triangle[length=1*\DTZU,width=1*\DTZU]}},
  {-{Triangle[length=1*\DTZU,width=1*\DTZU]}}
 },
 DECLARE.prec/.style={
  semithick,rounded corners,
  {-{Triangle[length=1*\DTZU,width=1*\DTZU]Circle[length=1*\DTZU,width=1*\DTZU]}},
  shorten >=-0.5*\DTZU
 },
 DECLARE.alt.prec/.style={
  semithick,rounded corners,
  postaction={draw, shorten >= 0.5*\DTZU, double distance=0.25*\DTZU, {-{Triangle[length=1*\DTZU,width=1*\DTZU]}}},
  {-{Circle[length=1*\DTZU,width=1*\DTZU]}},
  shorten >= -0.5*\DTZU
 },
 DECLARE.chn.prec/.style={
  semithick,rounded corners,
  preaction={draw, shorten >= 0.5*\DTZU, double distance=0.25*\DTZU, {-{Triangle[length=1*\DTZU,width=1*\DTZU]}}},
  {-{Circle[length=1*\DTZU,width=1*\DTZU]}},
  shorten >= -0.5*\DTZU
 },
 DECLARE.succ/.style={
  semithick,rounded corners,
  {Circle[length=1*\DTZU,width=1*\DTZU]}-{Triangle[length=1*\DTZU,width=1*\DTZU]Circle[length=1*\DTZU,width=1*\DTZU]},
  shorten <=-0.5*\DTZU,
  shorten >=-0.5*\DTZU
 },
 DECLARE.coex/.style={
  semithick,rounded corners,
  {Circle[length=1*\DTZU,width=1*\DTZU]}-{Circle[length=1*\DTZU,width=1*\DTZU]},
  shorten <=-0.5*\DTZU,
  shorten >=-0.5*\DTZU
 },
 DECLARE.alt.succ/.style={
  semithick,rounded corners,
  postaction={draw, shorten >= 0.5*\DTZU, shorten <= -0.5*\DTZU, double distance=0.25*\DTZU, {Circle[length=1*\DTZU,width=1*\DTZU]}-{Triangle[length=1*\DTZU,width=1*\DTZU]}},
  {-{Circle[length=1*\DTZU,width=1*\DTZU]}},
  shorten >= -0.5*\DTZU
 },
 DECLARE.chn.succ/.style={
  semithick,rounded corners,
  preaction={draw, shorten >= 0.5*\DTZU, shorten <= -0.5*\DTZU, double distance=0.25*\DTZU, {Circle[length=1*\DTZU,width=1*\DTZU]}-{Triangle[length=1*\DTZU,width=1*\DTZU]}},
  {-{Circle[length=1*\DTZU,width=1*\DTZU]}},
  shorten >= -0.5*\DTZU
 }
}
